Approximating Dynamic Time Warping and Edit Distance for a Pair of Point Sequences

We give the first subquadratic-time approximation schemes for dynamic time warping (DTW) and edit distance (ED) of several natural families of point sequences in $\mathbb{R}^d$, for any fixed $d \ge 1$. In particular, our algorithms compute $(1+\varepsilon)$-approximations of DTW and ED in time near-linear for point sequences drawn from k-packed or k-bounded curves, and subquadratic for backbone sequences. Roughly speaking, a curve is $\kappa$-packed if the length of its intersection with any ball of radius $r$ is at most $\kappa \cdot r$, and a curve is $\kappa$-bounded if the sub-curve between two curve points does not go too far from the two points compared to the distance between the two points. In backbone sequences, consecutive points are spaced at approximately equal distances apart, and no two points lie very close together. Recent results suggest that a subquadratic algorithm for DTW or ED is unlikely for an arbitrary pair of point sequences even for $d=1$. Our algorithms work by constructing a small set of rectangular regions that cover the entries of the dynamic programming table commonly used for these distance measures. The weights of entries inside each rectangle are roughly the same, so we are able to use efficient procedures to approximately compute the cheapest paths through these rectangles.

==> algorithm.tex <==

\section{Approximation Algorithm for DTW} \label{sec:alg}

Let $P = \langle p_1, \ldots, p_m \rangle$ and $Q = \langle q_1, \ldots, q_n
\rangle$ be two point sequences in $\R^d$, and let $\eps \in (0,1)$ be a
parameter.  We present a $(1+\eps)$-approximation algorithm for computing
$\dtw(P,Q)$.  Without loss of generality, assume that $m \le n$ and $\eps \ge
1/n$.  If $\eps < 1/n$, we can simply compute $\dtw(P,Q)$ in $O(mn) = O(n/\eps)$
time using straightforward dynamic programming.

For a pair of positive integers $i < i'$, let $[i:i'] = \{i, i+1, \ldots, i'\}$,
and let $[i] = [1:i]$.  Consider the weighted DAG $\G = (\V, \E)$ where $\V = \{
(i,j) \mid i \in [m], j \in [n] \}$ and each node $(i,j)$ is connected to the
nodes $(i+1, j)$, $(i, j+1)$, and $(i+1, j+1)$.  We define a weight function
$\wei: \V \rightarrow \R_{\ge 0}$ where $\wei(i,j) = ||p_i q_j||$.  We regard
$\V$ as a set of (integer) grid points in $\R^2$, and each edge in $\E$ is a
horizontal, vertical, or diagonal (slope 1) segment connecting its endpoints.
The endpoints of an edge will be referred to as \emph{neighbors} (or
\emph{neighboring points}).  Thus we regard $\G$ as a geometric graph embedded in
$\R^2$.  We set $s = (1,1)$ and $t = (m,n)$.

We call a polygonal curve $\pi$ connecting two points of $\V$ \emph{admissible} if
(i) $\pi$ is monotone in both $x$- and $y$-direction; (ii) $\pi$ consists of
horizontal, vertical, or diagonal segments; and (iii) the vertices of $\pi$
(i.e. the points at which it turns) are grid points.  We note that $\pi$ is
a path in $\G$.  We will not distinguish between the polygonal curve and the path
in $\G$.  Suppose $\pi = \langle u_1, u_2, \ldots, u_k \rangle$ in $\G$, then we
define the \emph{length} of $\pi$, $\ell(\pi)$, to be $k -1$, and its weight
$\wei(\pi)$ to be $\sum_{i=1}^{k-1} \wei(u_i)$; note that we do not include $\wei(u_k)$
in the sum.  The weight of an edge $(u_i, u_{i+1})$ in $\G$ is $\wei(u_i)$.
Let~$\pi[u,v]$ denote the subpath of~$\pi$ between points~$u$ and~$v$.

It is known that $\dtw(P,Q)$ is the minimum weight of an admissible path from
$s$ to $t$, and that it can be computed in $O(mn)$ time.  Our goal is to
estimate $\dtw(P,Q)$ within relative error $\eps$, without computing $\G$
explicitly.
We first give an overview of the algorithm and then describe each step in detail.
We define a \emph{rectangle}~$\rect = [i_1:i_2] \times [j_1:j_2]$ for $1 \leq i_1 \leq i_2 \leq
m,1 \leq j_1 \leq j_2 \leq n$, to be a rectangular subgrid of~$\V$, i.e., $\rect = \Set{(a,b) \mid
a \in [i_1:i_2],b \in [j_1:j_2]}$.
Rectangle~$\rect$ is called degenerate if~$i_1 = i_2$ or~$j_1 = j_2$.
The boundary of~$\rect$, denoted by~$\partial \rect$, is the set of points~$\partial \rect =
\Set{(a,b) \mid a = \Set{i_1,i_2}\text{ or }b = \Set{j_1,j_2}}$.
\begin{enumerate}[(i)]
  \item We compute a value $\dmin$ such that $\dmin \le \dtw(P,Q) \le 8n
    \dmin$.  

  \item Using the estimate~$\dmin$ and the error parameter~$\eps$, we partition~$\V$ into a
    family~$\rects$ of rectangles so that the weight of all points in each rectangle~$\rect$ is
    almost the same, say, roughly~$\lambda \rect$.
    Let~$\boundaries = \Cup_{\rect \in \rects} \partial \rect$ be the set of boundary points in
    the rectangles of~$\rects$.

    The sizes of~$\rects$ and~$\boundaries$ depend on how well behaved the curves~$\gamma_P$
    and~$\gamma_Q$ are.
    In the worst case~$|\rects|,|\boundaries| = \Theta(mn)$, but they are much smaller for many
    well-behaved curves such as $\kappa$-packed or $\kappa$-bounded curves.

  \item We order the rectangles in~$\rects$, say, $\rects = \langle \rect_1,\dots,\rect_\sigma
    \rangle$, so that if there is a path from~$s$ to a point in~$\rect_i$ that passes
    through~$\rect_j$ then~$\rect_j$ appears before~$\rect_i$.

  \item We set the \emph{costs} of all points in~$\rect \in \rects$ to~$\lambda \rect$.
    Let~$\lambda : \V \to \R_{\geq 0}$ be the resulting cost function.
    We compute the optimal paths from~$s$ to all points of~$\boundaries$ under the cost
    function~$\lambda$.
    \note{Make sure costs and weights are used correctly throughout.}
\end{enumerate}

We now describe steps (i)--(iv) in detail.

\paragraph{An $O(n)$ approximation.} 
Let $\dfr(P,Q)$ denote the discrete \frechet distance between $P$ and $Q$, i.e.,
replace sum with max in the definition of~$\dtw(P,Q)$.
\begin{lemma}
  $\displaystyle \dfr(P,Q) \le \dtw(P,Q) \le 2n \cdot \dfr(P,Q)$
  \label{lemma:n_approx}
\end{lemma}
\begin{proof}
  Let $C^*$ be the set of correspondences corresponding to $\dtw(P,Q)$.  Then
  $ \dfr(P,Q) \le \max_{(p,q) \in C^*} ||pq|| \le \sum_{(p,q) \in C^*} ||pq|| =
  \dtw(P,Q).$
  Similarly, let $\overline{C}$ be the set of correspondences corresponding to
  $\dfr(P,Q)$.  Then
  $ \dtw(P,Q) \le \sum_{(p,q) \in \overline{C}} ||pq|| \le 2n \max_{(p,q) \in
    \overline{C}} ||pq|| = 2n \dfr(P,Q)$.
    The second inequality follows because $|\overline{C}| \le m+n \le 2n$.
\end{proof}

Aronov \etal~\cite{AHKWW2006} gave a near-linear time algorithm for computing the
approximate discrete \frechet distance for point sequences drawn from
$\kappa$-bounded curves.  Their algorithm directly implies an $O(\kappa^d n\log
n)$-time 2-approximation algorithm for computing $\dfr(P,Q)$ for
$\kappa$-bounded curves.  It turns out that the same algorithm also works for
$\kappa$-packed curves.  More specifically, we just need to show that the number
of points in a $\mu$-simplified sequence (defined in Section~3.2 of
\cite{AHKWW2006}) in a ball $\ball$ of radius $\delta$ is bounded by $O(\kappa
\delta / \mu)$, and the rest of Section~3.3 of \cite{AHKWW2006} will follow.
Consider another ball $\ball'$ with the same center as $\ball$, but with a
radius $\delta+\mu$.  For every point of the simplified sequence inside $\ball$,
it is easy to see that there is a portion of the underlying curve of length at
least $\mu$ inside ball $\ball'$.  By $\kappa$-packedness, the total length of
the underlying curve inside $\ball'$ is $O(\kappa (\delta+\mu))$.  With $\mu =
O(\eps \delta)$, the total number of points in $\ball$ is bounded by $O(\kappa /
\eps)$.  Using the same grid idea for range search, a $2$-approximate discrete
\frechet distance for point sequences drawn from $\kappa$-packed curves can be
computed in $O(\kappa n \log n)$ time.  

Let $\overline{\dfr}(P,Q)$ be the 2-approximate discrete \frechet distance such
that $\dfr(P,Q) \le \overline{\dfr}(P,Q) \le 2\dfr(P,Q)$.  Set
$\dmin = \overline{\dfr}(P,Q)/2$, and we have 
  $\dmin \le \dtw(P,Q) \le 8n \dmin$.
Let $\dmax = 8n \dmin$.
\note{Why did we increase $\dmax$?}

\paragraph{Clustering algorithm.}
We cluster (partition) a subset of points of~$\V$ into a set~$\rects$ of rectangles and assign a
cost~$\lambda \rect$ to each rectangle~$\rect \in \rects$ so that the following property holds.
Let~$(i,j) \in \V$ be a point such that~$\wei(i,j) \leq \dmax$.
Then there is a rectangle~$\rect \in \rects$ such that $(i,j) \in \rect$ and
$$|\wei(i,j) - \lambda \rect| \leq \eps \max\Set{\wei(i,j),\dmin/2n}.$$

We describe in Section~\ref{sec:clustering} an efficient algorithm for constructing the
set~$\rects$ along with the cost function~$\lambda$.
Let~$\boundaries$ be the set of boundary points in the rectangles of~$\rects$.
Set~$\sigma = |\rects|$ and~$\beta = |\boundaries|$.

\paragraph{Ordering rectangles.}
We construct a directed graph~$\gH = (\gX,\gT)$ where~$\gX = [1:t]$ and~$(u,v)$, for~$1 \leq u
\neq v \leq \sigma$, is an edge in~$\gT$ if~$\rect_u$ and~$\rect_v$ have neighboring vertices,
i.e., there are boundary points~$p \in \rect_u$ and~$q \in \rect_v$ such that $(p,q) \in \E$.
We first write a few properties of~$\gH$.
We defer their proofs until after the last property is presented, because all three proofs are
nearly identical.
\begin{lemma}
  Graph~$\gH$ is acyclic.
  \label{lemma:acyclic}
\end{lemma}
\begin{lemma}
  Graph~$\gH$ is planar, and thus~$|\gT| = O(\sigma)$.
  \label{lemma:planar}
\end{lemma}
\begin{lemma}
  Let~$\rect_u,\rect_v \in \rects$ be two rectangles such that a path in~$\G$ from~$s$ to a point
  of~$\rect_v$ passes through a point of~$\rect_u$.
  There is a path from~$u$ to~$v$ in~$\gH$.
  \label{lemma:paths_through_rectangles}
\end{lemma}
\begin{proof}
  Consider the following algorithm for constructing~$\gH$.
  This algorithm is only used for the sake of proof; we give an~$O(\beta)$ time algorithm for
  constructing~$\gH$ below.

  \emph{Contracting} an edge~$(u,v)$ of a graph removes edges~$(u,v)$ from the graph, identifies
  vertices~$u$ and~$v$, and removes parallel edges created in the process.
  We construct graph~$\gH$ from~$\G$ by iteratively contracting edges in the following manner.
  Say vertex~$u$ (created by contractions) belongs to rectangle~$\rect \in \rects$ if all vertices
  of~$\G$ identified to~$u$ originally lied in~$\rect$.
  In each iteration, we contract a single edge~$(u,v)$ such that~$u$ and~$v$ both belong to the
  same rectangle~$\rect$.
  The process terminates when there are no such edges exist to contract.

  The vertices within any one rectangle~$\rect$ are all connected in~$\G$ through paths that stay
  within~$\rect$.
  Therefore, the process above does terminate after creating~$\gH$.
  Acyclicity, planarity, and strong connectivity are all maintained during edge contraction,
  proving the lemmas.
\end{proof}

Lemmas~\ref{lemma:acyclic} and~\ref{lemma:paths_through_rectangles} imply that a topological
ordering of vertices of~$\gH$ gives a desired ordering of rectangles in~$\rects$.
Namely, if a path in~$\G$ from~$s$ to a point of~$\rect_v$ passes through~$\rect_u$,
then~$\rect_u$ appears before~$\rect_v$ in the ordering.

We now describe an~$O(\beta)$ time algorithm for constructing~$\gH$.
We first sort all boundary vertices in the lexicographic order.
Let~$\boundaries_i$ be the sequence of boundary vertices that lie in column~$i$, i.e., whose
$x$-coordinate is~$i$, sorted in increasing order of their $y$-coordinates.
Let~$(i,j) \in \boundaries_i$ be a boundary point of a rectangle~$\rect_u$.
If~$(i,j)$ lies on the top boundary of~$\rect_u$ and~$(i,j+1)$ lies on the bottom boundary
of~$\rect_v$, then we add edge~$(u,v)$ to~$\gT$.
Similarly, if~$(i,j)$ lies on the right boundary of~$\rect_u$ and~$(i+1,j)$ lies on the left
boundary of~$\rect_w$, then we add the edge~$(u,w)$.
Note that if~$(i,j)$ lies both on the top and the right boundary of~$\rect_u$, then~$(i,j)$ is the
upper right vertex of~$\rect_u$.
In this case, if~$(i+1,j+1)$ is the bottom-left vertex of rectangle~$\rect_z$, then we also add
the edge~$(u,z)$.

The above step may add multiple edges between a pair of vertices, so we lexicographically sort the
edges we have added in~$O(\beta)$ time and remove duplicates.
\note{How do we sort them so quickly?}

The total time spent in constructing~$\gH$ is~$O(\beta)$.
In the next section, we describe the algorithm for computing the shortest paths from~$s$ to the
boundary vertices in~$\boundaries$.

\begin{figure}
  \centering
  \begin{tabular}{m{4cm}m{4cm}}
    \multicolumn{1}{c}{\includegraphics[height=3cm]{pictures/packed_curves.pdf}} &
    \multicolumn{1}{c}{\includegraphics[height=2cm]{pictures/top_snow.png}} \\
    \multicolumn{1}{c}{(a)} &
    \multicolumn{1}{c}{(b)}
  \end{tabular}
  \caption{(a) $\kappa$-packed curves that are not $\kappa$-bounded.
    (b) The top half of the Koch snowflake is a $\kappa$-bounded curve that is not
  $\kappa$-packed.}
  \label{fig:alg}
\end{figure}



==> analysis.tex <==
\section{Analysis} \label{sec:analysis}

In this section, we analyze the correctness and running time of our algorithm.  

\paragraph{Correctness.}
First, we show that the set of rectangles $\rects$ satisfies the conditions in step
(ii) of the algorithm.

\begin{lemma}
  The set of rectangles $\rects$ satisfies the following properties:
  \begin{enumerate}[(i)]
    \item for all $\rect \in \rects$ and $(i,j) \in \rect$, 
      $|\wei(i,j) - \wei_{\rect}| \le \eps \max\{ \wei_{\rect}, \dmin/2n\}$.

    \item if $(i,j) \in \V$ and $\wei(i,j) \le \dmax$, then there exists rectangle $\rect \in
      \rects$ such that $(i,j) \in \rect$. 
  \end{enumerate}
  \label{lemma:rectangle_property}
\end{lemma}
\begin{proof}
  Suppose $\rect$ is constructed from some well-separated pair $(u_t, v_t) \in \family$.
  By construction, if $(i,j) \in \rect$, then $p_i \in \hsq_{u_t}$ and $q_j \in
  \hsq_{v_t}$.  Therefore, $\wei(i,j) = ||p_i q_j|| \le \dsq(u_t, v_t) + 2\sqrt{2}
  (\Delta(u_t) + \Delta(v_t))$.  By property (P1) and $\wei_{\rect} = \dsq(u_t, v_t)$, 
  we have $\wei(i,j) \le \wei_{\rect} + 4\sqrt{2} \eps \max \{\wei_{\rect}, \dmin/2n \}$.
  By appropriate constant scaling of $\eps$, (i) is proved.
  We now prove (ii).  By property (P2), there must exist a pair $(u_t, v_t) \in \family$
  such that $p_i \in P_{u_t}$ and $q_j \in Q_{v_t}$.  It is easy to check that $(i,j)$ is
  in one of the rectangles constructed from $(u_t, v_t)$.
\end{proof}

We now show that the algorithm returns a $(1+\eps)$-approximation of $\dtw(P,Q)$.  
\begin{lemma}
  For each $(i,j) \in \boundaries$, if $\dtw(i,j) \le \dmax$, then $|\adtw(i,j) - 
  \dtw(i,j)| \le \eps \max\{\dtw(i,j), (i+j)\dmin/2n \} $.
  \label{lemma:correctness}
\end{lemma}
\begin{proof}
  We prove one direction $\adtw(i,j) - \dtw(i,j) \le \eps \max\{\dtw(i,j), (i+j)\dmin/2n
  \}$ by induction on $\boundaries$ using the same order the $\adtw$ values are computed.
  The other direction is similar.
  The lemma is obviously true for $(1,1)$.  Assume it is true for all points of
  $\boundaries$ before $(i,j)$, and we prove that it is also true for $(i,j)$.

  In the first case, $(i,j)$ does not hit any rectangle in $\rects$ and $\adtw(i,j)$ is computed using
  Eq.~(\ref{eq:compute_dtw1}).  Let $(a,b) \in \{ (i-1,j), (i, j-1), (i-1,j-1) \}$ be the
  predecessor of $(i,j)$ in the optimal admissible path from $(1,1)$ to $(i,j)$.
  Pair~$(a,b) \in \rect$ for some rectangle~$\rect$.
  Since~$(i,j)$ does not hit any rectangle, then~$(a,b)$ must actually lie on the boundary
  of~$\rect$.
  Since
  $\dtw(a,b) \le \dtw(i,j) \le \dmax$, we have $\adtw(a,b) - \dtw(a,b) \le \eps
  \max\{\dtw(a,b), (a+b)\dmin/2n\}$.  
  So $\adtw(i,j) - \dtw(i,j) = \adtw(a,b) - \dtw(a,b) \le \eps \max\{\dtw(a,b), (a+b)\dmin/2n\}
  \le \eps \max\{\dtw(i,j), (i+j)\dmin/2n\}$.

  In the second case, there exists some rectangle $\rect \in \rects$ hit by $(i,j)$ and
  $\adtw(i,j)$ is computed using Eq.~(\ref{eq:compute_dtw2}).  Let $\pi^*(i,j)$ denote the
  the optimal admissible path from $(1,1)$ to $(i,j)$.  Let $(a,b)$ be the intersection of
  $\pi^*(i,j)$ and the boundary of $\rect$.  If $(a,b) \in N_2$, we can modify the portion
  of $\pi^*(i,j)$ in $\rect$ such that it goes through the left-most point in $N_3$ and 
  increase the total weight by at most $\eps \max\{\dtw(i,j), (i+j)\dmin/2n\}$ (by
  Lemma~\ref{lemma:rectangle_property}).  So we assume $(a,b) \in N_1 \cup N_2$.  
  Then 
  \begin{align*}
    \adtw(i,j) &\le \adtw(a,b) + \max\{i-a, j-b\} \wei_{\rect} \\
    &\le \dtw(a,b) + \eps \max \{ \dtw(a,b), (a+b) \dmin/2n \} + \max\{i-a, j-b\} \wei_{\rect}\\
    & \le \dtw(i,j) + \eps \max \{ \dtw(i,j), (i+j) \dmin/2n \}.
  \end{align*}
\end{proof}
By Lemma~\ref{lemma:correctness}, $|\adtw(m,n) - \dtw(m,n)| \le \eps \max\{\dtw(m,n),
(m+n)\dmin/2n\} = \eps \dtw(m,n)$, i.e., our algorithm returns a $(1+\eps)$-approximation
of $\dtw(P,Q)$.


\paragraph{Running time.}
We show that the running time of our algorithm is subquadratic when the input
sequences are well-behaved.  

The running time of step (i) has been analyzed in Section~\ref{sec:alg_step1}, namely,
$O(\kappa n \log n)$, $O(\kappa^d n \log n)$ and $O(n^{2-2/d})$ time for $\kappa$-packed,
$\kappa$-bounded and protein backbone input sequences, respectively.  We first show that
the number of boundary points in $\boundaries$ is small in
Lemma~\ref{lemma:num_boundary_pts}.  Intuitively, the bounds follows from the fact that
well-behaved sequences do not enter and exit the square of any quadtree node too many
times.

\begin{lemma}
  The total number of boundary points of rectangles in $\rects$ is $O(\frac{\kappa}{\eps}
  n \log n)$ for $\kappa$-packed input sequences, $O(\frac{\kappa^d}{\eps^d}
  n \log n)$ for $\kappa$-bounded input sequences, and
	$O(\frac{1}{\eps} n^{2-1/d} \log n)$ for protein backbone curves..
  \label{lemma:num_boundary_pts}
\end{lemma}
\begin{proof}
  First, we consider the case for $\kappa$-packed sequences.  Fix some $i \in [m]$.  
  We bound the number of boundary points in the $i$-th column of $\V$.  We know that the active nodes are
  in $O(\log n)$ levels of the quadtree $\T$.
  Let~$u$ be a node such that~$p_i \in \hsq_u$.
  There are~$O(\log n)$ such nodes~$u$.
  By Lemma~\ref{lemma:wspd}, there exists some constant
  $c$ such that for any $v$ with
  $(u, v) \in \family$, $\sq_v$ is contained in a ball $\ball$ concentric with
  $\sq_{u}$ of radius $\frac{c}{\eps} \Delta(u)$.  By $\kappa$-packedness, the length 
  of the polygonal curve $\gamma_Q$ inside $\ball$ is at most $\kappa c
  \Delta(u)/\eps$ for some constant~$c$.
  We bound the number of maximal contiguous subsequences from
  $\hsq_v$'s with $(u, v) \in \family$.
  
  Consider any $(u, v) \in \family$.  There are two types of maximal
  contiguous subsequences of $\{j \mid q_j \in Q \cap \hsq_v \}$.  Most subsequences are
  of the first type where the first point of the subsequence lies inside $\sq_v$, and the
  point after the last point of the subsequence lies outside $\hsq_v$.  These subsequences
  use
  a portion of $\gamma_Q$ of length at least $\Delta(v)/2$.  The last subsequence may be
  of the second type if it contains the last point of $Q$ which lies inside $\hsq_v$.  Since
  $\hsq_v$ is contained in the union of $\sq_v$ and its $3^d-1$ neighbors in the same level of
  $\T$, every point on $\gamma_Q$ is used at most $3^d$ times.
  According to Lemma~\ref{lemma:wspd}(ii), we have~$\Delta(v) \geq \Delta(u)/2$.
  Therefore, the number of
  maximal contiguous subsequences of the first type is bounded by $(\kappa c \Delta(u)
  / \eps) * 3^d / (\Delta(v)/2) = O(\kappa/\eps)$.  For the second-type sequences, we
  bound the number of $v$'s such that $\hsq_v$ contains the last point of $Q$, $q_n$.  
  Suppose node $u$ is at level $t$ of the quadtree.
  By Lemma~\ref{lemma:wspd}(ii), such $v$'s can be from levels $t-1, t, t+1$.  In each level,
  $q_n$ can be in the $\hsq_v$ of at most $3^d$ $v$'s.  Thus, the number of maximal
  contiguous subsequences of the second type is at most $3^{d+1} = O(1)$.
  Summing over $O(\log n)$ $u$ such that $p_i \in \hsq_u$ and $i \in [m]$, 
  $|\boundaries|$ is bounded by $O(\frac{\kappa}{\eps} n \log n)$.

  Next, we prove the bound for $\kappa$-bounded sequences in a similar fashion.  Again, we
  bound the number of boundary points in the $i$-th column of $\V$.  Consider the same
  pair $(u, v) \in \family$.  We first show that for any two maximal contiguous
  subsequences $[y_1^-:y_1^+]$ and $[y_2^-:y_2^+]$, $||q_{y_1^-} q_{y_2^-}|| \ge
  \Delta(v)/(\kappa+2)$.  This is because between points $q_{y_1^-}$ and $q_{y_2^-}$, the
  curve $\gamma_Q$ goes from inside $\sq_v$ to outside $\hsq_v$ which spans
  distance at least $\Delta(v)/2$.  Let $q$ be the intersection of this portion of
  $\gamma_Q$ with the boundary of $\hsq_v$.  By $\kappa$-boundedness, $\gamma_Q(y_1^-:y_2^-) \subseteq
  \ball(q_{y_1^-}, \frac{\kappa}{2} ||q_{y_1^-} q_{y_2^-}||) \cup \ball(q_{y_2^-},
  \frac{\kappa}{2} ||q_{y_1^-} q_{y_2^-}||)$.  Therefore, $(1+\kappa/2) ||q_{y_1^-}
  q_{y_2^-}|| \ge ||q_{y_1^-} q|| \ge \Delta(v) /2$.  The claim follows.  By a packing
  argument, the number of maximal contiguous subsequences in $\hsq_v$ is bounded by $O(\kappa^d)$.
  Finally, there can be at most $O(1/\eps^d)$ $v$'s
	such that $(u, v) \in \family$
  by another packing argument on the ball $\ball$.  So the number of maximal contiguous
  subsequences in all $\hsq_v$'s with $(u, v) \in \family$ is $O(\kappa^d/ \eps^d)$.
  Again, summing over $O(\log n)$ $u$ such that $p_i \in \hsq_u$ and $i\in [m]$, we have $
  |\boundaries| = O(\frac{\kappa^d}{\eps^d} n \log n)$.
	
  To prove the bound for protein backbone sequences, we also consider two types of maximal 
  contiguous subsequences as for $\kappa$-packed sequences.  The bound for the second type
  is the same; so we focus on the first type.  Consider the same pair
  $(u, v) \in \family$. Using the same packing argument on the ball $\ball$, there
  can be at most $O(1/\eps^d)$ $v$'s such that $(u, v) \in \family$.  By the
  property that two consecutive points on a backbone curve have distance between
  $c_1$ and $c_2$, there must exist one point on any maximal contiguous subsequence of the
  first type that is at most $c_2$ away from the boundary of $\sq_v$. 
  The volumn of the region containing first points is $O(\Delta(v)^d -
  (\Delta(v) - c_2)^d) = O(\Delta(v)^{d-1})$.  Since any two points on the backbone
  curve $Q$ are at least distance $1$ apart, the maximum number of maximal
  contiguous subsequence in a node $v$ is $O(\Delta(v)^{d-1})$ using packing
  argument. Hence the number of maximal contiguous subsequences in all $\hsq_v$'s
  with $(u, v) \in \family$ is $O(\frac{\Delta(v)^{d-1}}{\eps^d})$. On the other
  hand, the last point of any maximal contiguous subsequence has to be at most $c_2$
  away from the boundary of $\hsq_v$.  Which means that the length of any maximal
  contiguous subsequence has to be at least $O(\Delta(v))$. Since there are a total
  of $m$ points in the backbone curve $Q$, the total number of maximal contiguous
  subsequences in all $\hsq_v$'s with $(u, v) \in \family$ is
  $O(\frac{m}{\Delta(v)})$.
	
  The total number of maximal contiguous subsequence in all $\hsq_v$'s with 
  $(u, v) \in \family$ is minimized when the two balancing terms are equal:
  $ \frac{\Delta(v)^{d-1}}{\eps^d} = (\frac{m}{\Delta(v)})$, which is equivalent to when 
  $\Delta(v) = \eps m^{1/d} $. The total number of maximal contiguous subsequence
  is thus $O(\frac{1}{\eps} m^{1-1/d})$.
  By summing over $O(\log n)$ $u$ such that $p_i \in \hsq_u$ and $i\in [m]$, 
  we have $|\boundaries| = O(\frac{1}{\eps} n^{2-1/d} \log n)$.
	
	
\end{proof}

By Lemma~\ref{lemma:num_boundary_pts}, the time to construct the family $\family$ of
well-separated pairs and the set $\rects$ of rectangles can be bounded by 
$O(\frac{\kappa}{\eps} n \log n)$ for $\kappa$-packed input sequences,
$O(\frac{\kappa^d}{\eps^d} n \log n)$ for $\kappa$-bounded input sequences, and
$O(\frac{1}{\eps} n^{2-1/d} \log n)$ for protein backbone sequences.

Using the range-min data structure described in Section~\ref{sec:alg}, step (iii) of the
algorithm can be completed in time $O(|\boundaries|)$.  In summary, we have the following
running times.

\begin{lemma}
  The running time of our algorithm is $O(\frac{\kappa}{\eps} n \log n)$ for $\kappa$-packed input
  sequences, $O(\frac{\kappa^d}{\eps^d} n \log n)$ for $\kappa$-bounded input
  sequences, and $O(\frac{1}{\eps} n^{2-1/d} \log n)$ for protein backbone input
  sequences, where $d$ is the dimension.
  \label{lemma:run_time}
\end{lemma}




==> clustering-deterministic.tex <==
\section{Clustering Algorithm} \label{sec:clustering}

First, we define $\mu$-simplification of a sequence.
\begin{definition}
  Given a sequence $Q = \langle q_1, \dots, q_n\rangle$ in $\R^d$, a
  subsequence $\tQ =
  \langle Q_{i_1}, \dots, Q_{i_k} \rangle$ is a \emph{left $\mu$-simplification} of
  $Q$ if 
  \begin{enumerate}[(i)]
    \item $1\le i_1 < i_2 < \dots < i_k\le n$
    \item for any integer $j \in (i_{t-1}, i_t)$, $d(q_j, q_{i_{t-1}}) \le \mu$.
    \item for any $t \in [2..k]$, we have $d(q_{i_{t-1}}, q_{i_t}) > \mu$.
  \end{enumerate}
  Similarly, $\tQ$ is a \emph{right $\mu$-simplification} if condition (ii)
  becomes: for any integer $j \in (i_{t-1}, i_t)$, $d(q_j, q_{i_t}) \le \mu$.
\end{definition}


\begin{lemma}
  A left or right $\mu$-simplification $\tQ$ of a sequence $Q$ of length $n$ in
  $\R^d$ can be computed in $O(n)$ time.
  \label{lemma:simp}
\end{lemma}
\begin{proof}
  A left $\mu$-simplification can be constructed in the following steps:
  \begin{enumerate}[(i)]
    \item add the first point $q_1$ to $\tQ$.
    \item greedily go throught the points of $Q$ in order, until the first point
      $q_i$ that is more than $\mu$ away from the previous added point, and add
      $q_i$ to $\tQ$; repeat until all points of $Q$ have been checked. 
  \end{enumerate}
  Clearly, the run time is $O(n)$.  A right $\mu$-simplification can be obtained
  similarly by going through the points of $Q$ in the opposite direction.
\end{proof}

We describe an algorithm for partitioning~$\V$ into a family of rectangles.

Let $\lmin = \lfloor \log_2 \frac{\eps \dmin}{2n} \rfloor$, $\lmax = \lceil \log_2
2\dmax\rceil$, $\rmin = 2^{\lmin}$, and $\rmax = 2^{\lmax}$.  Let $\H$ be an axis-aligned
hypercube that contains both $P$ and $Q$ and whose side length is $2^{\Delta}$,
for some integer $\Delta$, such that $2^{\Delta-1} \le \diam(P \cup Q) \le
2^{\Delta}$.  A quadtree $\T$ on $\H$ is a $2^d$-way tree, each of whose node $v$ is
associated with an axis-aligned box $\sq_v$.  If $v$ is the root of $\T$, then $\sq_v =
\H$.  The boxes associated with the children of a node $v$ are obtained by partitioning
$\sq_v$ into $2^d$ congruent hypercubes --- the side length of each resulting box is half
that of $\sq_v$.  If $v$ is a leaf, then the side length of $\sq_v$ is $\rmin$.
$\T$ induces a hierarchical grid inside $\H$ --- depth $i$ nodes partition $\H$ into a
$2^i \times 2^i$ uniform grid.  For a node $v \in \T$, let $\parent(v)$ denote its parent,
$\child(v)$ the set of children of $v$, $\Delta(v)$ the side length of $\sq_v$,
$P_v = P \cap \sq_v$, and $Q_v = Q \cap \sq_v$.  Set $m_v = |P_v|$ and
$n_v = |Q_v|$.  For two nodes $u,v \in \T$, let $\dsq(u,v) = \min_{p,q \in \sq_u\times
\sq_v} ||pq||$.  A node $v$ is called a \emph{neighboring} node of $u$ if $\Delta(u) =
\Delta(v)$ and $\dsq(u,v) = 0$, i.e., $\partial \sq_u \cap \partial \sq_v \neq
\varnothing$.

We call a node $v$ of $\T$ \emph{active} if $\Delta(v) \le \rmax$ and $m_v+n_v >
0$. Let $\Aset$ denote the
set of active nodes of $\T$. Set $\Aset$
corresponds to the bottom portion of $\T$ of height $\lmax =
O(\log(n/\eps)) = O(\log n)$.  By construction, $\sum_{v \in \Aset} m_v = O(m \log n)$ and
$\sum_{v \in \Aset} n_v = O(n \log n)$.
We only construct the active nodes of $\T$ and the sets $P_v, Q_v$ for all active
nodes.  This step takes a total of $O(n \log n)$ time (recall that $m \le n$).

The clustering algorithm works in two stages.  The first stage constructs a family
$\family = \Set{ (u_1,v_1), \ldots, (u_s, v_s)}$ of pairs of active nodes of $\T$ with the
following properties:
\bitem
    \item[(P1)] For every $t \le s$, $\max\Set{ \Delta(u_t), \Delta(v_t)} \le \eps \max\Set{
        \dsq(u_t, v_t), \dmin/2n}$.
    \item[(P2)] For all pairs $(i,j) \in [m] \times [n]$ with $||p_i q_j|| \le
        \dmax$, there is a unique index $t$ such that $p_i \in P_{u_t}$ and $q_j \in
        Q_{v_t}$.
\eitem

We now describe each stage in detail, prove the correctness of the algorithm, and
then analyze its performance for different families of curves.

\paragraph{First stage.}  The properties (P1) and (P2) are similar to those for the
so-called \emph{well-separated pair decomposition} (WSPD) of a point set, introduced by
Callahan and Kosaraju \cite{CK1995} (see also Har-Peled \cite{HP-book}).  We therefore adapt their
algorithm.  We first describe a recursive procedure \pair$(u,v)$, where $u,v$ are two
active nodes, which generates a family of pairs for $P_u, Q_v$.
\begin{center}
    \begin{tabular}{l}
        \hline
        \pair$(u,v)$ \\
        \textbf{if} $\max\Set{\Delta(u), \Delta(v)} \le \eps \max\Set{\dsq(u,v), \dmin/2n}$ \\
        ~ ~ add $(u,v)$ to $\family$; return \\
        \textbf{if} $\Delta(u) \ge \Delta(v)$, \textbf{then} \\
        ~ ~ $\forall w \in \child(u)$ ~ ~ \pair$(w,v)$ \\
        ~ ~ \textbf{else} $\forall z \in \child(v)$ ~ ~ \pair$(u,z)$ \\
        \hline
    \end{tabular}
\end{center}

Let $u_0$ be an active node with $\Delta(u_0) = \rmax$ and $P_{u_0} \neq
\varnothing$.  For every neighboring node $v_0$ of $u_0$ with $Q_{v_0} \neq
\varnothing$, we call \pair$(u_0, v_0)$.  

(P1) is obviously true by the termination condition of the \pair~procedure.  
(P2) is true because $p_i$ and $q_j$ are
contained in two neighboring active nodes of $\T$ in level $\lmax$ initially. 
By adapting the analysis of the WSPD algorithm, the following lemma
can be proven.
%Its proof is omitted because of lack of space.

\begin{lemma}
    If $(u,v) \in \family$, then
        (i) $\max\Set{\Delta(u), \Delta(v)} \le \min\Set{ \Delta(\parent(u)),
            \Delta(\parent(v))}$; (ii)
        $\Delta(u)/2 \le \Delta(v) \le 2\Delta(u)$; and
        (iii) there is a constant $c \ge 0$ such that $\dsq(u,v) \le \frac{c}{\eps}
            \Delta(u)$.
    %\begin{enumerate}[(i)]
        %\item $\max\Set{\Delta(u), \Delta(v)} \le \min\Set{ \Delta(\parent(u)),
            %\Delta(\parent(v))}$;
        %\item $\Delta(u)/2 \le \Delta(v) \le 2\Delta(u)$; and
        %\item there is a constant $c \ge 0$ such that $\dsq(u,v) \le \frac{c}{\eps}
            %\Delta(u)$.
    %\end{enumerate}
    \label{lemma:wspd}
\end{lemma}

The running time of the first stage is $O(n \log n + s)$.

\paragraph{Second stage.}
Define $\underline{h}$ as lowest level in $\T$ where an active node is present, and 
$\bar{h}$ as the highest level in $\T$ where an active node is present, satisfying 
$1 \le \underline{h} \le \bar{h} \le \Delta$.
As a pre-processing step, for each level where at least an active node
is present, i.e., $i \in [\underline{h} \ldots \bar{h}]$, we compute a 
$\epsilon 2^i$-simplification. $\bar{h} - \underline{h} = O(\log n)$ since $A$ corresponds to the
bottom portion of $\T$ of height $O(\log n)$. By \ref{lemma:simp}, the total time spent on 
simplifying the curves on 
$\bar{h} - \underline{h}$ levels is thus $O(n \log n)$.

Fix a pair $(u,v) \in \family$.
We have computed an $\epsilon \Delta(v)$-simplification on the $Q$, which intersects with $v$.
We define $\tilde{P}_u$ as any point in $P_u$ or any point that $\epsilon \Delta(u)$-simplifies 
to a point in $P_u$.

This allows us to define the distance between active nodes $\tilde{\dsq}(u, v)$ after simplification 
to be the maximum distance between any point in $\tilde{P}_u$, 
and any point in $\tilde{Q}_v$.
We define the $\tilde{\Delta}(u)$ after simplification similarly by the 
maximum distance between two points that are in $\tilde{P}_u$. 
By definition of simplification,
\begin{equation}
\tilde{\dsq}(u, v) \le \dsq(u, v) + 2\epsilon \Delta(v)
\end{equation}
\begin{equation}
\tilde{\Delta}(u) \le \Delta(u) + 2\epsilon \Delta(v)
\end{equation}
The above relationship implies that the property (P1) and \ref{lemma:wspd} still hold for the new
distance functions $\tilde{\dsq}$ and $\tilde{\Delta}$ for all active nodes. However, the property
(P2) no longer holds since a point $q_j$ belonging to the node $v_{t'}$ could be simplified into $v_t$
if $\dsq(v_{t'}, v_t) < \epsilon \Delta(v_t)$. Hence there could exist two different indices 
$t'$ and $t$ such that both $\tilde{Q}_{v_{t}}$ and $\tilde{Q}_{v_{t'}}$ contain $q_j$ 
after simplification.

Let $[x_1^{-}:x_1^{+}],\dots,[x_{\mu_u}^{-}:x_{\mu_u}^{+}]$ be the maximal contiguous subsequences
of~$\Set{i \mid p_i \in \tilde{P}_u}$.
Similarly, let $[y_1^{-}:y_1^{+}],\dots,[y_{\nu_v}^{-}:y_{\nu_v}^{+}]$ be the maximal contiguous
subsequences of~$\Set{j \mid q_j \in \tilde{Q}_v}$.
For every pair $a \in [1:\mu_u], b \in [1:\nu_v]$, we generate the rectangle $[x_a^{-}:x_a^{+}]
\times [y_b^{-}:y_b^{+}]$.
The total number of rectangles generated is $\mu_u \nu_v$, and the total number of their boundary
vertices is $2m_u \nu_v + 2\mu_u n_v$.

We repeat the above procedure for all pairs in~$\family$.
Let~$\rects$ be the set of rectangles generated and~$\boundaries$ be the set of their boundary
vertices, i.e., $\boundaries = \Cup_{\rect \in \rects} \partial \rect$.
We have~$|\rects| = \sum_{i=1}^s \mu_{u_i} \nu_{v_i}$ and~$\beta = |\boundaries| = \sum_{i=1}^s
2(m_{u_i} \nu_{v_i} + \mu_{u_i} n_{v_i})$.
The total time spent in generating~$\rects$ is~$O(|\rects|)$.

\paragraph{Third stage.}
Since the property (P2) no longer holds, the rectangles in $\rects$ could overlap with each other,
hence the algorithm described in \ref{sec:alg} is not directly applicable. In this stage, given the
set of rectangles, we perform a trapezoidal decomposition of the rectangles into rectangles that 
are disjoint, while only increasing $|\rects|$ and $\beta$ by a constant factor.

The following 3 cases could happen when the rectangles overlap each other in the dynamic programming
matrix, shown in \ref{fig:rect_overlap}:
  \begin{enumerate}[(i)]
    \item One rectangle is fully contained inside another rectangle.
		\item Two rectangles cross each other
    \item Two rectangles overlap in one or two corners
  \end{enumerate}
	\begin{figure}
  \centering
  \begin{tabular}{m{4cm}m{4cm}m{4cm}}
    \multicolumn{1}{c}{\includegraphics[height=3cm]{pictures/overlap_case1}} &
		\multicolumn{1}{c}{\includegraphics[height=3cm]{pictures/overlap_case3}} &
    \multicolumn{1}{c}{\includegraphics[height=3cm]{pictures/overlap_case2}} \\
    \multicolumn{1}{c}{(a)} &
    \multicolumn{1}{c}{(b)}
  \end{tabular}
  \caption{(a) containment (b) crossing each other
    (c) partial overlapping }
  \label{fig:rect_overlap}
\end{figure}

In the first case, the smaller rectangle fully contained in the larger rectangle is removed from 
$\rects$, since the larger rectangle ensures the similarity of weights for all points within.

In the second case, trapezoidal decomposition adds extra two vertical segments that decomposes the
rectangle with smaller height into 3 distinct rectangles. Two extra rectangles created are attributed
to the rectangle with larger height; two extra segments of boundary points are also attributed to
the rectangle with larger height. The total number of increased boundary points is thus no greater
than the boundary points on the vertical segments of the rectangle with larger height.

In the third case, trapezoidal decomposition adds extra one vertical segment that decomposes the 
rectangle with smaller height into 2 distinct rectangles. One extra rectangle created is attributed
to the rectangle with larger heigher; one extra segments of boundary points is also attributed to 
that rectangle. Thus the number of points added per rectangle
is no greater than the boundary points on the vertical segments of the rectangle.

\begin{lemma}
  Vertical trapezoidal decomposition of the overlapping rectangles into rectangles that only overlap
	at boundaries increases $|\rects|$ and $\beta$ by a constant factor.
\end{lemma}

\begin{lemma}
  If $P,Q$ are sequences drawn from $\kappa$-packed curves in $\R^d$, then $\sum_{z \in N(w)}
  \lambda_z^{+} =
  O(\frac{\kappa}{\eps} \Delta(w))$.
  \label{lemma:curve-within-ball}
\end{lemma}
\begin{proof}
  By Lemma~\ref{lemma:wspd}, $\dsq(w,z) \leq \frac{c}{\eps}\Delta(w)$ for all $z \in N(w)$ before
  we performed the postprocessing step to ensure $z \in \T_{h-1}$ for some~$h$.
  Since $\Delta(z) = 2\Delta(w)$, the cells associated with $N(w)$ are contained in the ball
  $\ball_w$ of radius $\rho_w = (\frac{c}{\eps} + 3\sqrt{d})\Delta(w)$ centered at the center of
  $\sq_w$.
  Since we assume $\xi \in [0: \Delta(w) - 1]^d$, we have $\Delta(z) + \xi \subset \ball_w^{+}$
  where $\ball_w^{+}$ is the ball of radius $\rho_w + \sqrt{d}\Delta(w)$ concentric with
  $\ball_w$.
  \note{Check radii.}

  Curve~$\gamma_Q$ being $\kappa$-packed implies that $|\gamma_Q \cap B_w^{+}| \le \kappa(\rho_w +
  \sqrt{d}\Delta(w)) = O(\frac{\kappa}{\eps} \Delta(w))$.
  Since~$\Delta(\sq_z^{+}) = 3 \Delta(\sq_z)$ for any $z \in N(w)$, each point
  inside~$\ball_w^{+}$ is covered by at most~$3^d$ $\sq_z^{+}$'s.
  Hence,
  $$\sum_{z \in N(w)} \lambda_w^{+} \le 3^d |\gamma_Q \cap \ball_w^{+}| = O(\frac{\kappa}{\eps}
  \Delta(w))$$
  as claimed.
\end{proof}

Lemmas~\ref{lemma:length-bound} and~\ref{lemma:curve-within-ball} along with~\eqref{eq:mw-sum}
imply that
\begin{align*}
  \E[\Q_h(\xi)] &\leq \sum_{w \in \treeC_h} m^+_w \sum_{z \in N(w)} \E[\nu_z(\xi)] \leq \sum_{w \in
  \treeC_h}m_w^{+} \sum_{z \in N(w)} \frac{2d \lambda_z^{+}}{\Delta(w)} \\
  &\leq \sum_{w \in \treeC_h} m_w^{+} \cdot O(\frac{\kappa}{\eps}) = O(\frac{\kappa}{\eps}m).
\end{align*}

Since $\lmax = O(\log n)$, we have $\E[\Q(\xi)] = O(\frac{\kappa}{\eps} m \log n)$.
This completes the proof of Lemma~\ref{lemma:packed-Q}.
Putting everything together, we obtain the following.

\begin{lemma}
  If $P,Q$ are sequences drawn from $\kappa$-packed curves in $\R^d$, where $d \ge 1$ is a
  constant, then~$\V$ can be partitioned, in $O(\frac{\kappa}{\eps} n \log n)$ expected time, into
  a set of pairwise-disjoint rectangles such that the expected number of vertices
  is~$O(\frac{\kappa}{\eps} n \log n)$.
\end{lemma}



==> clustering.tex <==
\section{Clustering Algorithm} \label{sec:clustering}

In this section, we describe an algorithm for partitioning~$\V$ into a family of rectangles.

Let $\lmin = \lfloor \log_2 \frac{\eps \dmin}{2n} \rfloor$, $\lmax = \lceil \log_2
2\dmax\rceil$, $\rmin = 2^{\lmin}$, and $\rmax = 2^{\lmax}$.
For simplicity, we assume $\lmin = 0$ and $\rmin = 1$.
Then, $\lmax = O(\log n)$.
Let $\H_0$ be an axis-aligned
hypercube that contains both $P$ and $Q$ and whose side length is $2^{\Delta}$,
for some integer $\Delta$, such that $2^{\Delta-1} \le \diam(P \cup Q) \le
2^{\Delta}$.
Suppose $\H_0 = \Prod_{i=1}^d [x_i - 2^\Delta, x_i]$.
Then we set $\H_1 = \Prod_{i=1}^d [x_i - 2^{\Delta+1}, x_i]$.
For simplicity, we assume $\H_1 = [0, 2^{\Delta+1}]^d$.
Let $\H^{+} = [0,2^{\Delta+2}]^d$.
For $i \in [1:d]$, we choose a value $\xi_i \in [0:2^\Delta - 1]$ uniformly at random.
Set $\xi = (\xi_1,\dots,\xi_d)$ and $\H = \H_1 + \xi$.
A quadtree $\T$ on $\H$ is a $2^d$-way tree, each of whose node $v$ is
associated with an axis-aligned box $\sq_v$.  If $v$ is the root of $\T$, then $\sq_v =
\H$.  The boxes associated with the children of a node $v$ are obtained by partitioning
$\sq_v$ into $2^d$ congruent hypercubes --- the side length of each resulting box is half
that of $\sq_v$.  If $v$ is a leaf, then the side length of $\sq_v$ is $\rmin$.
$\T$ induces a hierarchical grid inside $\H$ --- depth $i$ nodes partition $\H$ into a
$2^i \times 2^i$ uniform grid.  For a node $v \in \T$, let $\parent(v)$ denote its parent,
$\child(v)$ the set of children of $v$, $\Delta(v)$ the side length of $\sq_v$,
$P_v = P \cap \sq_v$, and $Q_v = Q \cap \sq_v$.  Set $m_v = |P_v|$ and
$n_v = |Q_v|$.
For a hypercube~$\sq$, let~$\#(P \cap \sq)$ denote the number of maximal contiguous subsequences
of~$P \cap \sq$.
Similarly define~$\#(Q \cap \sq)$.
We set $\mu_v = \#(P \cap \sq_v)$ and $\nu_v = \#(Q \cap \sq_v)$.
For two nodes $u,v \in \T$, let $\dsq(u,v) = \min_{p,q \in \sq_u\times
\sq_v} ||pq||$.  A node $v$ is called a \emph{neighboring} node of $u$ if $\Delta(u) =
\Delta(v)$ and $\dsq(u,v) = 0$, i.e., $\partial \sq_u \cap \partial \sq_v \neq
\varnothing$.

We call a node $v$ of $\T$ \emph{active} if $\Delta(v) \le \rmax$ and $m_v+n_v >
0$. Let $\Aset$ denote the
set of active nodes of $\T$. Set $\Aset$
corresponds to the bottom portion of $\T$ of height $\lmax =
O(\log(n/\eps)) = O(\log n)$.  By construction, $\sum_{v \in \Aset} m_v = O(m \log n)$ and
$\sum_{v \in \Aset} n_v = O(n \log n)$.
We only construct the active nodes of $\T$ and the sets $P_v, Q_v$ for all active
nodes.  This step takes a total of $O(n \log n)$ time (recall that $m \le n$).

The clustering algorithm works in two stages.  The first stage constructs a family
$\family = \Set{ (u_1,v_1), \ldots, (u_s, v_s)}$ of pairs of active nodes of $\T$ with the
following properties:
\bitem
    \item[(P1)] For every $t \le s$, $\max\Set{ \Delta(u_t), \Delta(v_t)} \le \eps \max\Set{
        \dsq(u_t, v_t), \dmin/2n}$.
    \item[(P2)] For all pairs $(i,j) \in [m] \times [n]$ with $||p_i q_j|| \le
        \dmax$, there is a unique index $t$ such that $p_i \in P_{u_t}$ and $q_j \in
        Q_{v_t}$.
\eitem

We now describe each stage in detail, prove the correctness of the algorithm, and
then analyze its performance for different families of curves.

\paragraph{First stage.}  The properties (P1) and (P2) are similar to those for the
so-called \emph{well-separated pair decomposition} (WSPD) of a point set, introduced by
Callahan and Kosaraju \cite{CK1995} (see also Har-Peled \cite{HP-book}).  We therefore adapt their
algorithm.  We first describe a recursive procedure \pair$(u,v)$, where $u,v$ are two
active nodes, which generates a family of pairs for $P_u, Q_v$.
\begin{center}
    \begin{tabular}{l}
        \hline
        \pair$(u,v)$ \\
        \textbf{if} $\max\Set{\Delta(u), \Delta(v)} \le \eps \max\Set{\dsq(u,v), \dmin/2n}$ \\
        ~ ~ add $(u,v)$ to $\family$; return \\
        \textbf{if} $\Delta(u) \ge \Delta(v)$, \textbf{then} \\
        ~ ~ $\forall w \in \child(u)$ ~ ~ \pair$(w,v)$ \\
        ~ ~ \textbf{else} $\forall z \in \child(v)$ ~ ~ \pair$(u,z)$ \\
        \hline
    \end{tabular}
\end{center}

Let $u_0$ be an active node with $\Delta(u_0) = \rmax$ and $P_{u_0} \neq
\varnothing$.  For every neighboring node $v_0$ of $u_0$ with $Q_{v_0} \neq
\varnothing$, we call \pair$(u_0, v_0)$.  

(P1) is obviously true by the termination condition of the \pair~procedure.  
(P2) is true because $p_i$ and $q_j$ are
contained in two neighboring active nodes of $\T$ in level $\lmax$ initially. 
By adapting the analysis of the WSPD algorithm, the following lemma
can be proven.
%Its proof is omitted because of lack of space.

\begin{lemma}
    If $(u,v) \in \family$, then
        (i) $\max\Set{\Delta(u), \Delta(v)} \le \min\Set{ \Delta(\parent(u)),
            \Delta(\parent(v))}$; (ii)
        $\Delta(u)/2 \le \Delta(v) \le 2\Delta(u)$; and
        (iii) there is a constant $c \ge 0$ such that $\dsq(u,v) \le \frac{c}{\eps}
            \Delta(u)$.
    %\begin{enumerate}[(i)]
        %\item $\max\Set{\Delta(u), \Delta(v)} \le \min\Set{ \Delta(\parent(u)),
            %\Delta(\parent(v))}$;
        %\item $\Delta(u)/2 \le \Delta(v) \le 2\Delta(u)$; and
        %\item there is a constant $c \ge 0$ such that $\dsq(u,v) \le \frac{c}{\eps}
            %\Delta(u)$.
    %\end{enumerate}
    \label{lemma:wspd}
\end{lemma}

The running time of the first stage is $O(n \log n + s)$.

\paragraph{Second stage.}
Fix a pair $(u,v) \in \family$.
Let $[x_1^{-}:x_1^{+}],\dots,[x_{\mu_u}^{-}:x_{\mu_u}^{+}]$ be the maximal contiguous subsequences
of~$\Set{i \mid p_i \in P_u}$.
Similarly, let $[y_1^{-}:y_1^{+}],\dots,[y_{\nu_v}^{-}:y_{\nu_v}^{+}]$ be the maximal contiguous
subsequences of~$\Set{j \mid q_j \in Q_v}$.
For every pair $a \in [1:\mu_u], b \in [1:\nu_v]$, we generate the rectangle $[x_a^{-}:x_a^{+}]
\times [y_b^{-}:y_b^{+}]$.
The total number of rectangles generated is $\mu_u \nu_v$, and the total number of their boundary
vertices is $m_u \nu_v + \mu_u n_v$.

We repeate the above procedure for all pairs in~$\family$.
Let~$\rects$ be the set of rectangles generated and~$\boundaries$ be the set of their boundary
vertices, i.e., $\boundaries = \Cup_{\rect \in \rects} \partial \rect$.
We have~$|\rects| = \sum_{i=1}^s \mu_{u_i} \nu_{v_i}$ and~$\beta = |\boundaries| = \sum_{i=1}^s
(m_{u_i} \nu_{v_i} + \mu_{u_i} n_{v_i})$.
The total time spent in generating~$\rects$ is~$O(|\rects|)$.
\note{Not~$O(\beta)$?}

\paragraph{Analysis.}
The value of~$\beta$ depends on the shift~$\xi$ used to construct the quad tree~$\T$, and we
use~$\beta(\xi)$ to express this dependence.
Recall that~$\xi$ is chosen randomly.
We prove a bound on~$\E[\beta(\xi)]$, the expected value of~$\beta$.
Let $\Q(\xi) = \sum_{i=1}^s m_{u_i} \nu_{v_i}$.
We prove the following.
\begin{lemma}
  If $P,Q$ are sequences drawn from $\kappa$-packed curves in $\R^d$, then $\E[\Q(\xi)] =
  O(\frac{\kappa}{\eps} m \log n)$.
  \label{lemma:packed-Q}
\end{lemma}

A similar argument implies that the expected value of $\sum_{i=1}^s \mu_{u_i} n_{v_i}$ is
$O(\frac{\kappa}{\eps} n \log n)$, from which we conclude:
\begin{corollary}
  If $P,Q$ are sequences drawn from $\kappa$-packed curves in $\R^d$, then $\E[\beta(\xi)] =
  O(\frac{\kappa}{\eps} n \log n)$.
\end{corollary}

We now prove Lemma~\ref{lemma:packed-Q}.
For a node $u \in \T$, let $N(u) = \Set{v \mid (u,v) \in \family}$.
Fix a pair $(u,v) \in \family$.
By Lemma~\ref{lemma:wspd}, $\Delta(u) / 2 \le \Delta(v) \le 2 \Delta(u)$.
For simplicity, assume that $\Delta(v) = \Delta(u)/2$.
If $\Delta(v) = \Delta(u)$ or $\Delta(v) = 2\Delta(u)$, we replace $(u,v)$ with
$(u,v_1),\dots,(u,v_\gamma)$ where $v_1,\dots,v_\gamma$ are the children or grand-children of~$v$
depending on whether $\Delta(v) = \Delta(u)$ or $\Delta(v) = 2\Delta(u)$.
This step does not decrease the value of~$\beta(\xi)$ for any~$\xi$.
For $h \in [0:\lmax]$, let~$\T_h$ be the set of nodes of~$\T$ at height~$h$.
Since $m_u = 0$ for all $u \in \T_h \setminus A$, we can write
\begin{align*}
  \Q(\xi) &= \sum_{i=1}^s m_{u_i} \nu_{v_i} = \sum_{u \in A} m_u \sum_{v \in N(u)} \nu_v \\
          &= \sum_{h=0}^{\lmax} \sum_{u \in \T_h} m_u \sum_{v \in N(u)} \nu_v =
  \sum_{h=0}^{\lmax}
  \Q_h(\xi),
\end{align*}
where $\Q_h(\xi) = \sum_{u \in \T_h} m_u \sum_{v \in N(u)} \nu_v$.

In the following, we bound~$\E[\Q_h(\xi)]$.

\begin{lemma}
  Let $\xi = (\xi_1,\dots,\xi_d) \in [0:2^\Delta - 1]$, and let $\xihat = (\xi \mod 2^h, \dots,
  \xi_d \mod 2^h)$.
  Then $\Q_h(\xi) = \Q_h(\xihat)$.
  \label{lemma:xihat}
\end{lemma}
\begin{proof}
  Let $\Sigma_{\xi} = \Set{\sq_w \mid w \in \T_h \cup \T_{h-1} \wedge (m_w > 0 \vee \nu_w > 0)}$.
  Similarly define $\Sigma_{\xihat}$.
  Because the cells of the nodes in $\T_h$ (resp. $\T_{h-1}$) form a uniform grid of size~$2^h$
  (resp.~$2^{h-1}$), translating the grid by a multiple of~$2^h$ along any axis does not have any
  impact as long as it continues to cover~$P \cup Q$.
  Since these conditions are true for~$\xi$ and~$\xihat$, we can conclude that $\Sigma_{\xi} =
  \Sigma_{\xihat}$, which implies the lemma.
\end{proof}

In view of Lemma~\ref{lemma:xihat}, to bound $\E[\Q_h(\xi)]$, we assume that $\xi$ is chosen
randomly from $[0:2^h - 1]^d$, with uniform distribution.
Recall that $\H = \H_0 + \xi$.
Suppose we construct a quad tree~$\treeC$ on~$\H_0$.
Then~$\T$ is a ``translate'' of~$\treeC$ by~$\xi$.
Abusing the notation a little, we use~$\sq_w$ to denote the hypercube associated with a node~$w$
of~$\treeC$.
Suppose $\sq_w = x_w + C_{\Delta(w)}$, where $C_r = [0,r]^d$.
We set $\sq_w^{+} = x_w + C_{2^h}$.
Let $m_w^{+} = |\sq_w^{+} \cap P|$ and $\lambda_w^{+} = |\curve_Q \cap \sq_w^{+}|$.
Let~$\treeC_h$ denote the set of node of~$\treeC$ at height~$h$.
Then there is a bijection between the nodes of~$\treeC_h$ and~$\T_h$, and for every $u \in \T_h$,
there is a node~$\tilde{u} \in \treeC_h$ such that $\sq_u = \sq_{\tilde{u}} + \xi$ and $\sq_u
\subseteq \sq_{\tilde{u}}^+$ for any $\xi \in [0,2^h - 1]$.
It is easy to verify that
\begin{equation}
\sum_{w \in \treeC_h} m_w^{+} \leq 2^d \sum_{w \in \treeC_h} m_w.
\label{eq:mw-sum}
\end{equation}
\note{Is this the right equation?}

We observe that for any node $u \in \T_h$, set~$N(u)$ does not depend on~$\xi$ in the sense that
$\Set{\sq_v \mid v \in N(u)} = \Set{\sq_z + \xi \mid z \in N(\tilde{u})}$ where~$\tilde{u} \in
\treeC_h$ is the node corresponding to~$u$ and~$N(\tilde{u})$ is the set of nodes
in~$\treeC_{h-1}$ that would pair with~$\tilde{u}$ if we run \pair~on~$\H_0$ (and ensure that all
neighbors of~$u$ belong to~$\treeC_{h-1}$).
For each $z \in \treeC_{h-1}$, we define $\nu_z(\xi) = \#(Q \cap (\sq_z + \xi))$.
Then we can rewrite $\Q_h(\xi) \leq \sum_{w \in \treeC_h} m_w^{+} \sum_{z \in N(w)} \nu_z(\xi)$.
Since $m_w^{+}$ and $N(w)$ are independent of~$\xi$, we have $\E[\Q_h(\xi)] \leq \sum_{w \in
\treeC_h} m_w^{+} \sum_{z \in N(w)} \E[\nu_z(\xi)]$.

\begin{lemma}
  $$\E[\nu_z(\xi)] \leq \frac{d \lambda_z^{+}}{\Delta(z)}.$$
  \label{lemma:length-bound}
\end{lemma}
\begin{proof}
  The value of~$\nu_z(\xi)$ is bounded by $|\gamma_Q \cap \partial (\sq_z + \xi)|$.
  Let~$f$ be the bottom facet of~$\sq_z$ in the $x_d$-direction.
  We show that the expected value of $|\gamma_Q \cap (f + \xi)|$ is at most
  $\frac{\lambda_z^+}{\Delta(z)}$.

  Let~$f^+$ be the bottom facet of~$\sq_z^{+}$ in the $x_d$-direction.
  We have~$f \subseteq f^+$.
  For $t \in [0:2^h - 1]$, let $\Q_f(t) = |\gamma_Q \cap (f^+ + (0,\dots,0,t))|$.
  Then for any $\xi = (\xi_1,\dots,\xi_d) \in [0:2^h - 1]^d$, we have $|\gamma_Q \cap (f + \xi)|
  \leq \Q_f(\xi_d)$.

  Let~$I$ be the extent of~$\sq_z^{+}$ along the $x_d$-axis; $|I| = 2\Delta(z)$.
  Let~$\eta$ be the projection of $\gamma_Q \cap \sq_z^{+}$ onto the $x$-axis; $|\eta| \le
  \lambda_z^{+}$.
  For any $t \in I$, let $\nu(t)$ denote the multiplicity of~$\eta$ at~$t$ such that $\nu(t) =
  |\gamma_Q \cap (f^+ + (0,\dots,0,t))|$.
  \note{Is this last expression correct? I'm not sure if we really need to project.}
  We have
  $$\E[\Q_f(t)] = \frac{1}{|I|} \int_{I} \nu(t) \dt = \frac{1}{2\Delta(z)} |\eta| \leq
  \frac{\lambda_z^{+}}{2\Delta(z)}.$$
  Repeating this argument for all $2d$ facets of~$\sq_z$, we obtain the desired bound on
  $\E[\nu_z(\xi)]$.
  \note{I think $I$ should be a set of integers and the final equations should be taken over a
  sum.}
\end{proof}

\begin{lemma}
  If $P,Q$ are sequences drawn from $\kappa$-packed curves in $\R^d$, then $\sum_{z \in N(w)}
  \lambda_z^{+} =
  O(\frac{\kappa}{\eps} \Delta(w))$.
  \label{lemma:curve-within-ball}
\end{lemma}
\begin{proof}
  By Lemma~\ref{lemma:wspd}, $\dsq(w,z) \leq \frac{c}{\eps}\Delta(w)$ for all $z \in N(w)$ before
  we performed the postprocessing step to ensure $z \in \T_{h-1}$ for some~$h$.
  Since $\Delta(z) = 2\Delta(w)$, the cells associated with $N(w)$ are contained in the ball
  $\ball_w$ of radius $\rho_w = (\frac{c}{\eps} + 3\sqrt{d})\Delta(w)$ centered at the center of
  $\sq_w$.
  Since we assume $\xi \in [0: \Delta(w) - 1]^d$, we have $\Delta(z) + \xi \subset \ball_w^{+}$
  where $\ball_w^{+}$ is the ball of radius $\rho_w + \sqrt{d}\Delta(w)$ concentric with
  $\ball_w$.
  \note{Check radii.}

  Curve~$\gamma_Q$ being $\kappa$-packed implies that $|\gamma_Q \cap B_w^{+}| \le \kappa(\rho_w +
  \sqrt{d}\Delta(w)) = O(\frac{\kappa}{\eps} \Delta(w))$.
  Since~$\Delta(\sq_z^{+}) = 3 \Delta(\sq_z)$ for any $z \in N(w)$, each point
  inside~$\ball_w^{+}$ is covered by at most~$3^d$ $\sq_z^{+}$'s.
  Hence,
  $$\sum_{z \in N(w)} \lambda_w^{+} \le 3^d |\gamma_Q \cap \ball_w^{+}| = O(\frac{\kappa}{\eps}
  \Delta(w))$$
  as claimed.
\end{proof}

Lemmas~\ref{lemma:length-bound} and~\ref{lemma:curve-within-ball} along with~\eqref{eq:mw-sum}
imply that
\begin{align*}
  \E[\Q_h(\xi)] &\leq \sum_{w \in \treeC_h} m^+_w \sum_{z \in N(w)} \E[\nu_z(\xi)] \leq \sum_{w \in
  \treeC_h}m_w^{+} \sum_{z \in N(w)} \frac{2d \lambda_z^{+}}{\Delta(w)} \\
  &\leq \sum_{w \in \treeC_h} m_w^{+} \cdot O(\frac{\kappa}{\eps}) = O(\frac{\kappa}{\eps}m).
\end{align*}

Since $\lmax = O(\log n)$, we have $\E[\Q(\xi)] = O(\frac{\kappa}{\eps} m \log n)$.
This completes the proof of Lemma~\ref{lemma:packed-Q}.
Putting everything together, we obtain the following.

\begin{lemma}
  If $P,Q$ are sequences drawn from $\kappa$-packed curves in $\R^d$, where $d \ge 1$ is a
  constant, then~$\V$ can be partitioned, in $O(\frac{\kappa}{\eps} n \log n)$ expected time, into
  a set of pairwise-disjoint rectangles such that the expected number of vertices
  is~$O(\frac{\kappa}{\eps} n \log n)$.
\end{lemma}



==> ed.tex <==
\section{Edit distance} \label{sec:ED}
We now show how our algorithm can be extended to compute the edit distance between $P$ and $Q$.
We define DAG $\G$ as before, except now $\V = \Set{(i,j) | i \in [m+1], j \in [n+1]}$.
We set $s = (1,1)$ and $t = (m+1,n+1)$.
For $i < m+1$ and $j < n+1$, we have~$\wei(i,j) = ||p_i q_j||$.
Otherwise~$\wei(i,j)$ is undefined.
For each horizontal or vertical edge~$e = (u_i,u_{i+1})$ in~$\G$, we have~$\wei(e) = g$.
Otherwise,~$\wei(e) = \min\Set{\wei(u_i),2g}$ to represent the two choices of adding a pair to
the edit distance correspondence or taking two gap penalties.
For an admissible path~$\pi = \langle u_1,u_2,\dots,u_k\rangle$, we have~$\ell(\pi) = k-1$ as
before, and $\wei(\pi) = \sum_{i=1}^{k-1} \wei((u_i,u_{i+1}))$.

If $m = n$, then we compute the cost of the monotone path~$\pi = \langle(1,1),
(2,2),\dots,(n+1,n+1)\rangle$.
If~$\wei(\pi) \leq g$, then it is returned as the optimal path.
Otherwise, we continue using the general scheme for DTW.
We set~$\dmin = g$ and $\dmax = 2(m + n)g$.
The same clustering scheme to compute~$\rects$ is used.
We define the cost $\lambda \rect$ of rectangle $\rect$ to be the weight of any one of its points.
It is now the case that if~$(i, j) \in \V$ has~$\wei(i,j) \leq \dmax$, then there is a rectangle
$\rect \in \rects$ such that $(i,j) \in \rect$ and
$$|\wei(i,j) - \lambda \rect| \leq \eps \max\Set{\wei(i,j),\dmin/(2(n+))}.$$
Rectangles are ordered as before.

For each horizontal or vertical edge~$e \in \E$, we set its cost~$\lambda(e) = g$.
For each diagonal edge~$e = (u,v) \in \E$ with $u \in \rect_u$, we set its cost $\lambda(e) =
\min\Set{\lambda \rect_u, 2g}$.
The main change from the previous algorithm is in computing cheapest paths to boundary vertices
under the cost function~$\lambda$.
The time complexity and approximation ratio analysis of the edit distance algorithm is the same as
in DTW.
We now show how to compute cheapest paths to the boundary vertices in~$\boundaries$.

For a point~$p \in \V$, again let~$\chi(p)$ be the minimum cost of a path in~$\G$ from~$s$ to~$p$
under the cost function~$\lambda$.
We only describe the algorithm for computing~$\chi(p)$ for all~$p \in \boundaries$.

Initially, we set~$\chi(s) = 0$.
We process the rectangles of~$\rects$ in the computed order.
Suppose we have processed~$\rect_1,\dots,\rect_{u-1}$, i.e. we have computed~$\chi(p)$ for all~$p
\in \boundaries_{u-1} = \Cup_{i=1}^{u-1} \partial \rect_i$.
Let ${\rect_u = [a^{-}:a^{+}] \times [b^{-}:b^{+}]}$ be the next rectangle in~$\rects$.
Without loss of generality, assume that~$a^{+}-a^{-} \ge b^{+}-b^{-}$.
Computing~$\chi(\cdot)$ for left and bottom boundaries is done as before using the new cost
function, so we focus on right and top boundaries.

It is no longer the case that the cost of a path~$\pi$ through rectangle~$\rect_u$ is
simply~$\ell(\pi) \lambda \rect_u$.
Let~$\ell^{\bot}(\pi)$ be the number of horizontal or vertical edges in~$\pi$ and
let~$\ell^{/}(\pi)$ be the number of diagonal edges so that~$\ell(\pi) = \ell^{\bot}(\pi) +
\ell^{/}(\pi)$.
We have~$\lambda(\pi) = \ell^{\bot}(\pi) \cdot g + \ell^{/}(\pi) \lambda \rect_u$.
We have~$\lambda \rect_u \leq 2g$, so cheapest admissible paths between vertices on~$\partial
\rect_u$ still maximize the number of diagonal edges used.
For a point~$p \in \rect_u$, define~$N(p)$ as before.
For a pair of points $p = (i,j)$ and $q = (i',j')$ in $\rect_u$ with $i' \ge i$ and $j' \ge j$,
let $d^{\bot}(p,q) = \max\Set{i' - i - (j' - j), j' - j - (i' - i)}$ and $d^{/} = \min\Set{i' - i,
j' - j}$.
For any point~$p$ on the right or top boundary of~$\rect_u$,
$$\chi(p) = \min_{q \in N(p)} \chi(q) + d^{\bot}(q, p) \cdot g + d^{/}(q,p) \lambda \rect_u.$$

\paragraph{Right boundary.}
For~$j \in [b^{-}:b^{+}]$, let~$p_j = (a^{+}, j)$ be a point on the right boundary of~$\rect_u$.
We partition~$N(p_j)$ into three sets.
\begin{enumerate}[(i)]
  \item $N_1(p_j) = \Set{(a^{-},l) \mid l \in [b^{-}:j]}$.
    For all points~$q \in N_1(p_j)$, we have~$d^{\bot}(q,p_j) = a^{+} - a^{-} - (j - l)$ and
    $d^{/}(q,p_j) = j - l$.
    For~$j \in [b^{-}:b^{+}]$, let~$Q_j = \min_{l \leq j} \chi(a^{-},l) + (a^{+} - a^{-} - (j -
    l))g + (j - l) \lambda \rect_u$.
    Therefore,
    $$\min_{q \in N_1(p_j)} \chi(q) + d^{\bot}(q, p_j) \cdot g + d^{/}(q,p_j) \lambda \rect_u =
    Q_j.$$

  \item $N_2(p_j) = \Set{(i,b^{-}) \mid i \in [a^{-}:a^{+} - (j-b^{-})]}$.
    There is a shortest path from~$q \in N_2(p_j)$ consisting of the horizontal segment $q
    \bar{p}_j$, where $\bar{p}_j = (a^{+} - j + b^{-},b^{-})$, and the diagonal $\bar{p}_j p_j$.
    Hence,
    $$\min_{q \in N_2(p_j)} \chi(q) + d^{\bot}(q, p_j) \cdot g + d^{/}(q,p_j) \lambda \rect_u =
    \chi(\bar{p_j}) + (j-b^{-}) \lambda \rect_u.$$

  \item $N_3(p_j) = \Set{(i,b^{-}) \mid i \in [a^{+} - j + b^{-} + 1:b^{+}]} \cup \Set{(a^{+},l
    \mid l \in [b^{-}:j)}$.
    There is a shortest path from ${q \in N_3(p_j)}$ to~$p_j$ consisting of the (possibly empty)
    diagonal from~$q$ followed by a vertical segment on the right boundary of~$\rect_u$.
    In particular, it passes through~$p_{j-1}$.
    Hence,
    $$\min_{q \in N_3(p_j)} \chi(q) + d^{\bot}(q, p_j) \cdot g + d^{/}(q, p_j) \lambda \rect_u=
    \chi(p_{j-1}) + g.$$
\end{enumerate}

Putting everything together,
\begin{align*}
\chi(p_j) &= \min_{q \in N(p_j)} \chi(q) + d^{\bot}(q, p_j) \cdot g + d^{/}(q, p_j) \lambda
  \rect_u\\
  &= \min\Set{Q_j,\chi(\bar{p}_j) + (j-b^{-}) \lambda \rect_u, \chi(p_{j-1}) + g}.
\end{align*}

Note that for any fixed $l \in [a^{-}:a^{+}]$, the value $\chi(a^{-},l) + (a^{+} - a^{-} - (j -
l))g + (j - l) \lambda \rect_u$ changes as~$j$ increases.
However, it always changes by exactly~$\lambda \rect_u - g$ every time~$j$ increases by~$1$.
Therefore, we can still compute~$Q_j$ for all $j \in [b^{-}:b^{+}]$ by making a single pass
through the left boundary of~$\rect_u$ in a total of~$O(b^{+} - b^{-})$ time.
After having computed~$Q_j$'s,~$\chi(p_j)$ can be computed in~$O(1)$ time each.

\paragraph{Top boundary.}
For $i \in [a^{-}:a^{+}]$, let $p_i = (i, b^{+})$ be a point on the top boundary of~$\rect_u$.
There are two cases whether the diagonal segment passing through~$p_i$ intersects the left or the
bottom boundary of~$\rect_u$, i.e. whether $i \le b^{+} - b^{-} + a^{-}$.
\paragraph{Case: $i \le a^{-} + (b^{+} - b^{-})$.}
This case is symmetric to the right boundary case.
We partition~$N(p_i)$ into three parts.
\begin{enumerate}[(i)]
  \item $N_1(p_i) = \Set{(a^{-}, j) \mid j \in [b^{-} + 1:b^{+} - i + a^{-}]}$.
    For $q \in N_1(p_i)$, there is a shortest path from~$q$ to~$p_i$ that passes
    through~$p_{i-1}$.
    Hence,
    $$\min_{q \in N_1(p_i)} \chi(q) + d^{\bot}(q, p_i) \cdot g + d^{/}(q, p_i) \lambda \rect_u = \chi(p_{i-1}) + g.$$

  \item $N_2(p_i) = \Set{(a^{-}, j) \mid j \in [b^{-}:b^{+} - i + a^{-}]}$.
    For $q \in N_2(p_i)$, there is a shortest path from~$q$ to~$p_i$ that passes through
    $\bar{p}_i = (a^{-}, b^{+} - i + a^{-})$, the intersection point of the diagonal through~$p_i$
    with the left boundary of~$\rect_u$.
    Hence,
    $$\mid_{q \in N_2(p_i)} \chi(q) + d^{\bot}(q, p_i) \cdot g + d^{/}(q, p_i) \lambda \rect_u =
    \chi(\bar{p}_i) + (i - a^{-}) \lambda \rect_u.$$

  \item $N_3(p_i) = \Set{(l, b^{-}) \mid l \in [a^{-}, i]}$.
    For any $q \in N_3(p_i)$, we have $d^{\bot}(q,p_i) = (b^{+}-b^{-} - (i-l))$ and $d^{/}(q,p_i)
    = i - l$.
    Let $\psi_i = \min_{a^{-} \le l \le i} \chi(l, b^{-}) + (b^{+} - b^{-} - (i - l)) \cdot g + (j
    - l) \lambda \rect_u $.
    We have
    $$\min_{q \in N_3(p_i)} \chi(q) + d^{\bot}(q, p_i) \cdot g + d^{/}(q, p_i) \lambda \rect_u =
    \psi_i.$$
\end{enumerate}

Hence,
$$\chi(p_i) = \min\Set{\chi(p_{i-1}) + g, \chi(\bar{p}_i) + (i-a^{-}) \lambda
\rect_u, \psi_i}.$$

As for the right boundary, after computing~$\psi_i$, for $i \in [a^{-}: a^{-} + (b^{+} - b^{-})]$,
we can compute~$\chi(p_i)$, for each $i \in [a^{-}:a^{-} + (b^{+} - b^{-})]$ in~$O(1)$ time each.

\paragraph{Case: $i > a^{-} + (b^{+} - b^{-})$.}
We partition~$N(p_i)$ into two sets.
\begin{enumerate}[(i)]
  \item $N_1(p_i) = \Set{(a^{-},j) \mid j \in [b^{-}:b^{+}]} \cup \Set{(l,b^{-}) \mid l \in
    [a^{-}:i-b^{+} + b^{-} - 1]} \cup {(l,b^{+}) \mid l \in [a^{-}:i-1]}$.
    For all $q \in N_1(p_i)$, there is a shortest path from~$q$ to~$p_i$ that passes
    through~$p_{i-1}$.
    Hence,
    $$\min_{q \in N_1(p_i)} \chi(q) + d^{\bot}(q, p_i) \cdot g + d^{/}(q, p_i) \lambda \rect_u =
    \chi(p_{i-1}) + g.$$
  \item $N_2(p_i) = \Set{(l,b^{-}) \mid l \in [i - b^{+} - b^{-}:i]}$.
    For all $q \in N_2(p_i)$, we have $d^{\bot}(q,p_i) = b^{+} - b^{-} - (i - l)$ and
    $d^{/}(q,p_i) = i - l$.
    Therefore, $$\min_{q \in N_2(p_i)} \chi(q) + d^{\bot}(q, p_i) \cdot g + d^{/}(q, p_i) \lambda
    \rect_u = \tilde{\psi}_i$$ where $\tilde{\psi}_i = \min_{q \in N_2(p_i)} \chi(q) + (b^{+} -
    b^{-} - (i - l)) \cdot g + (i - l) \lambda \rect_u$.
\end{enumerate}

Hence,
$$\chi(p_i) = \min\Set{\chi(p_{i-1}) + g, \tilde{\psi}_i}.$$
Again, for $i > a^{-} + (b^{+} - b^{-})$, we have $N_2(p_{i+1}) = (N_2(p_i) \cup \Set{(i+1,
b^{-})}) \setminus \Set{(i - b^{+} - b^{-}, b^{-})}$.
We maintain a subsequence $Q = \langle p_{i1}, \dots, p_{ir} \rangle$ of items such that (i)
$\chi(p_{i l}) + (b^{+} - b^{-} - (i - il)) \cdot g + (i - il) \lambda
\rect_u < \chi(p_{i(l + 1)}) + (b^{+} - b^{-} - (i - i(l+1))) \cdot g + (i - i(l+1)) \lambda
\rect_u$ for $1 \le l \le r$, and (ii) for all $b \in [il+1:j(l+1) -
1]$, we have $\chi(p_b) + (b^{+} - b^{-} - (i - b)) \cdot g + (i - b) \lambda
\rect_u \ge \chi(p_{i(l+1)}) + (b^{+} - b^{-} - (i - i(l+1))) \cdot g + (i - i(l+1)) \lambda
\rect_u$.
Then, $\tilde{\psi}_i = \chi(p_{i1}) + (b^{+} - b^{-} - (i - i1)) \cdot g + (i - i1) \lambda
\rect_u$.
For any~$p_b$, the value $\chi(p_b) + (b^{+} - b^{-} - (i - b)) \cdot g + (i - b) \lambda
\rect_u$ changes by exactly $\lambda \rect_u - g$ whenever~$i$ increases by~$1$.
Therefore, we can maintain sequence~$Q$ using nearly the same procedure as done for DTW.

When we process~$p_{i+1}$, we remove~$p_{i1}$ from~$Q$ if~$i1 = i + 1 - b^{+} - b^{-}$.
Next, we scan~$Q$ backwards and remove the current item~$p_{il}$ being scanned if
$$\chi(p_{il}) + (b^{+} - b^{-} - (i - il)) \cdot g + (i - il) \lambda \rect_u \geq
\chi((i+1,b^{-})) + (b^{+} - b^{-}) \cdot g.$$
Finally, we insert $(i+1,b^{-})$ into~$Q$ as its last item.
The time spent in updating~$Q$ while processing~$p_i$ is~$O(1+\kappa_i)$ where~$\kappa_i$ is the
number of items deleted from~$Q$ while processing~$p_i$.
Since each item is deleted at most once, the total running time is~$O(a^{+} - a^{-})$.

Putting everything together, the total time spent processing~$\rect_u$ is~$O(|\partial \rect_u|)$.
Hence, we conclude the following.
\begin{lemma}
  The total time spent in computing~$\chi(p)$ for all points $p \in \boundaries$ is~$O(\beta)$.
\end{lemma}

\paragraph{Acknowledgement.} The authors would like to thank Sariel Har-Peled for helpful comments
on an earlier version of this paper.
%
%\begin{shortversion}
%A detailed proof of Lemma~\ref{lemma:ed_approx} appears in the full version; we describe
%the high level ideas behind the proof.
%
%We begin by converting~$\sPi$ into~$\Pi_1$ such that if $u,v \in \E$ are two consecutive sampled
%entries on $\Pi_1$, then $\Pi_1(u,v)$ consists of zero or more vertical and diagonal segments
%followed by several horizontal and vertical segments (a staircase).
%In order to do so, we repeatedly find consecutive pairs of entries $u,v \in \E$ from $\sPi$ that
%violate this requirement, and move their initial diagonal and vertical segments left until the
%condition is satisfied or they hit another member of~$\E$.
%See Figure~\ref{fig:convert}(c).
%
%A similar surgery is performed to construct~$\Pi_2$ from~$\Pi_1$ so that between any two
%consecutive sampled entries~$u$ and~$v$ on~$\Pi_2$, path~$\Pi_2(u,v)$ consists of a single
%diagonal segment followed by several horizontal and vertical segments 
%(Figure~\ref{fig:convert}(d)).
%We create~$\Pi_2$ by moving diagonals of~$\Pi_1$ upward instead of to the left.
%
%Finally, we convert~$\Pi_2$ into~$\tPi$ by moving diagonal segments of~$\Pi_2$ horizontally
%or vertically to meet the diagonal edges in graph~$\H$.
%Afterward, for each pair of consecutive sampled entries~$u$ and~$v$ on~$\tPi$, we replace
%the horizontal and vertical segments at the end of~$\tPi(u,v)$ with a staircase walking down the
%diagonal~$\tau$ that initially separated~$u$ from~$v$ in the construction of~$\H$.
%Now~$\tPi(u,v)$ contains a single orthogonal segment to an entry~$w_1$, a diagonal segment ending
%in a staircase, and another orthogonal segment starting at entry~$w_2$.
%See Figure~\ref{fig:convert}(e).
%Replacing~$\Pi(w_1,w_2)$ with the cheapest set of diagonal and horizontal-vertical steps
%along~$\tau$ can only decrease its cost.
%The edges of~$G$ are weighted to approximate such cheapest paths.
%\begin{proof}
%
%We begin by converting~$\sPi$ into~$\Pi_1$ such that each pathlet of~$\Pi_1$ contains a no
%diagonal segments after the first horizontal segment.
%
%
%if $u,v \in \E$ are two consecutive sampled
%entries on $\Pi_1$, then $\Pi_1(u,v)$ consists of zero or more vertical and diagonal segments
%followed by several horizontal and vertical segments (a staircase).
%See
%Figure~\ref{fig:convert}(a).
%
%
%Finally, we convert~$\Pi_2$ into~$\tPi$ (see Figure~\ref{fig:ed}(c)).
%
%\begin{lemma}
%  $\Pi_2$ can be transformed to another admissible path $\tPi$ from $s$ to
%  $t$ such that $\wei(\tPi) \le (1+2\eps)^3 \wei(\Pi_1)$ and $\tPi$ is a path in
%  $\gH$.
%  \label{lemma:ed_approx2}
%\end{lemma}
%\begin{proof}
%Let $u = (i_u,j_u)$ and $v = (i_v, j_v)$ be two consecutive sampled entries on $\Pi_2$, and
%suppose $i_v - i_u \leq j_v - j_u$.
%In other words, the rectangle bound by $u$ and $v$ is wider than it is tall.
%Let~$\tau$ be the first diagonal lying between $u$ and $v$ inclusive when constructing graph~$\H$.
%We move the diagonal segment of~$\Pi_2(u,v)$ horizontally toward~$\tau$ until it reaches~$\tau$ or
%another sampled entry~$w$. We repeat this process until no moves are available.
%Similarly, we use vertical movements if $i_v - i_u > j_v - j_u$.
%After one such movement,~$\Pi_2$ may no longer have the structure promised above, i.e.,
%starting with a diagonal segment followed by orthogonal segments between every two consecutive sampled entries.
%However, if we create a new pair of sampled entries along the path during a horizontal movement,
%then they will still be in a wide configuration.
%Similarly, pairs created during vertical movements will still be in a tall configuration.
%So the process of moving diagonal segments toward dividing diagonals can continue.
%Each diagonal segment may be moved several
%times during the process, but it moves either always horizontally or always vertically.
%
%When the diagonal movements are complete, we perform one last change to create~$\tPi$.
%For any two consecutive sampled entries~$u$ and~$v$ on our path, we take the final set of
%horizontal and vertical segments leading to~$v$ and have them walk down the first diagonal~$\tau$ lying
%between~$u$ and~$v$ in a staircase fashion until the first Steiner entry on
%$\tau$ projected from $v$, and reach $v$ via a last orthogonal segment reaching $v$.
%%\note{Make a figure with non-trivial horizontal segments before the diagonal and after the staircase.}
%Changing the location of the horizontal and vertical steps has no effect on the cost
%of~$\tPi$.
%We use a similar projection argument to account for the changing cost of diagonal steps.
%As when creating~$\Pi_1$ and~$\Pi_2$, the entries of~$\tPi$ that moved horizontally
%from~$\Pi_2$ can be projected horizontally to distinct entries of~$\Pi_2$ without encountering
%other sample entries.
%Entries of~$\tPi$ that moved vertically from~$\Pi_2$ can be projected vertically.
%We have $\wei(\tPi) \le (1+2\eps)^3 \wei(\sPi)$.
%\end{proof}
%
%Now, consider any consecutive pair of sample entries~$u$ and~$v$ on~$\tPi$.
%Path~$\tPi(u,v)$ consists of a single orthogonal segment from $u$ to an entry~$w_1$, a
%diagonal segment ending with a staircase along the same diagonal until some entry
%$w_2$, and a single orthogonal segment from $w_2$ to $v$.
%The first and last orthogonal segments correspond to two orthogonal edges in $\H$.  The
%diagonal portion between $w_1$ and $w_2$ corresponds to a sequence of diagonal edges in
%$G$.  
%We can replace~$\tPi(w_1,w_2)$ with the cheapest combination of diagonal and
%horizontal-vertical steps, to obtain $\hPi$, without increasing the cost of~$\tPi$.
%Using a similar analysis as Lemma~\ref{lemma:ed_wei_approx}, we conclude
%$\wei(\hPi) \le (1+2\eps) \wei(\tPi) \le (1+2\eps)^4 \wei(\sPi)$.
%\end{proof}
%\end{shortversion}

%\usetikzlibrary{positioning}
%\tikzset{main node/.style={circle,fill=black!20,draw,minimum size=0.2cm,inner sep=0pt},}
%\begin{figure}
%\centering
%\begin{tabular}{ccc}
    %\includegraphics[height=3cm]{pictures/ed1.pdf} &
    %\includegraphics[height=3cm]{pictures/ed2.pdf} &
    %\includegraphics[height=3cm]{pictures/ed3.pdf} \\
    %(a) step 1 & (b) step 2 & (c) step 3
%\end{tabular}
%\caption{Steps of constructing $\tilde{\Pi}$ from $\Pi$ between two consecutive sampled
%entries $u,v$.  In each step, the red dotted curve represents the resulting path of this step.}
%\label{fig:ed}
%\end{figure}

\begin{comment}
\begin{theorem}
    Let $\A, \B$ be two point sequences of length at most $n$ drawn from $\kappa$-packed
    curves in $\R^d$.
  There exists an $O(\frac{\kappa^2}{\eps} n \log^2 n)$ time approximation scheme to
  compute $\ed(\A,\B)$.
\end{theorem}
\begin{theorem}
    Let $\A, \B$ be two point sequences of length at most $n$ drawn from $\kappa$-bounded
    curves in $\R^d$.
  There exists an $O(\frac{\kappa^d}{\eps^d} n \log^2 n)$ time approximation scheme to
  compute $\ed(\A,\B)$.
\end{theorem}

We want to show that the lemma \ref{lemma:approx} holds similarly for edit distance.


\begin{proof}
  The first step is to massage $\Pi$ such that if $u, v$ are two consecutive sampled entries on $\Pi$, the path on $\Pi$ between $u, v$ consists of two parts: the diagonal path segment followed by a horizontal and vertical segment (staircase) as shown in figure \ref{fig:ed_path_segment}. This can be done because of the following facts:


  \begin{enumerate}
  \item If $\Pi$ consists of a sequence consecutive horizontal and vertical segments, we can collapse the sequence of segments into one horizontal and one vertical segment as shown in figure \ref{fig:ed_observation1} without increasing $\ed$, since each horizontal/vertical step incur the same cost $g$, and the number of horizontal/vertical steps is the same for all L1 paths that have edge that goes downwards or to the right only.
    \begin{figure}
    \centering
    \begin{tikzpicture}
    
      \begin{scope}[xshift=4cm]
        \node[main node] (1) {};
        \node[main node] (2) [below = 1cm of 1]  {};
        \node[main node] (3) [right = 2cm of 2]  {};
        \node[main node] (4) [below = 2cm of 3] {};
        \node[main node] (5) [right = 1cm of 4] {};
        \node[main node] (6) [right = 3.2cm of 1] {};
    
        \path[->]
         (1) edge node {} (2)
             edge [dashed] node {} (6)
         (2) edge node {} (3)
         (3) edge node {} (4)
         (4) edge node {} (5)
         (6) edge [dashed] node {} (5)
        ;
        
      \end{scope}
        
    \end{tikzpicture}
    \caption{Collapse consecutive horizontal and vertical segments without increasing $\ed$}
    \label{fig:ed_observation1}
    \end{figure}
    
  \item The dashed path $\Pi'$ in figure \ref{fig:ed_observation2} has total cost at most $(1+\eps) \Pi$, provided that there is no sample point in the region enclosed by the two paths, since corresponding entry on $\Pi$ and $\Pi'$ differs in ratio by at most $(1+\eps)$.
  \begin{figure}
    \centering
    \begin{tikzpicture}
    
      \begin{scope}[xshift=4cm]
        \node[main node] (1) {};
        \node[main node] (2) [below = 1cm of 1]  {};
        \node[main node] (3) [below right = 1cm and 1cm of 2]  {};
        \node[main node] (7) [above = 1cm of 3]  {};
        \node[main node] (4) [right = 5cm of 1] {};
        \node[main node] (5) [right = 1cm of 4] {};
        \node[main node] (6) [below right = 1cm and 1cm of 5] {};
        \node[main node] (8) [left = 1cm of 6]  {};
    
        \path[->]
         (1) edge node {} (2)
             edge [dashed] node {} (7)
         (2) edge node {} (3)
         (7) edge node {} (3)
         
         (4) edge node {} (5)
             edge [dashed] node {} (8)
         (5) edge node {} (6)
         (8) edge [dashed] node {} (6)
        ;
        
      \end{scope}
        
    \end{tikzpicture}
    \caption{Switch diagonal segment with horizontal/vertical segments}
    \label{fig:ed_observation2}
    \end{figure}
    
  
  \end{enumerate}
  
  Based on the two observations, one can produce the path $\Pi_1$ that satisfies our requirement by the following steps:
  
  \begin{enumerate}
  \item collapse consecutive horizontal and vertical segments using the first observation
  \item move diagonal segments to the $u$ end by applying the second observation at most twice for each segment (when a horizontal and a vertical segment precede the diagonal segment). This makes the resulting curve a $(1+\eps)^2$ approximation of $\Pi$. After this there exists only one diagonal segment with $u$ as one of its end point.
  \item Collapse the remaining horizontal and vertical segments following the diagonal segments by the first observation.
  \end{enumerate}
  
  During the series of movements, whenever a sample point $u'$ is encountered, we use the similar strategy of making the curve pass through $u'$ and repeat the process for sub-intervals $(u, u')$ and $(u', v)$.
   
   The second step of massaging $\Pi_1$ into $\tilde{\Pi}$ that uses only edges from $G$ can be achieved using the same procedure described in \ref{fig:convert}. It is still valid that moving the diagonal horizontally to the left and right will not change the path value by more than $(1+\eps)$ as long as it does not encounter a sampled entry in the process because of observation 2. If a sampled entry is encountered, we split the path at that sampled entry and apply the same movement process for each segment.
\end{proof}

Without loss of generality, assume that there are more horizontal steps in the path than vertical steps in the path $\Pi$. Rearrange the staircase so that it consists of a diagonal path, an alternating set of horizontal and vertical steps, followed by a consecutive horizontal segment to the sampled point $v$, as shown in \ref{ed:diagonal}. Now treat the alternating horizontal and vertical steps as diagonal, and apply the second step in lemma \ref{lemma:approx}, we can produce $\tilde{\Pi}$ that uses only nodes in the constructed graph. The only difference is that at some step on the differentiating diagonal $\tau$ that separates $u$ and $v$, one can choose to change the path from going diagonally to going in a staircase fashion.

Since there is always an edge in our constructed graph between a sampled point and its horizontal and vertical projection to the diagonals (steiner points), and between two steiner points on the same diagonal, this path is contained in the constructed graph.
\begin{figure}
    \centering
    \begin{tikzpicture}        
      \begin{scope}[xshift=4cm]
        \node[main node] (1) {};
        \node[main node] (2) [below right = 3cm and 3cm of 1]  {};
        \node[main node] (3) [right = 0.5cm of 2]  {};
        \node[main node] (4) [below = 0.5cm of 3]  {};
        \node[main node] (5) [right = 0.5cm of 4] {};
        \node[main node] (6) [below = 0.5cm of 5] {};
        \node[main node] (7) [right = 1.5cm of 6] {};
    
        \path[->]
         (1) edge node {} (2)
         (2) edge node {} (3)
         (3) edge node {} (4)
         (4) edge node {} (5)
         (5) edge node {} (6)
         (6) edge node {} (7)
        ;
        
      \end{scope}
        
    \end{tikzpicture}
    \caption{near optimal path on the diagonal $\tau$}
    \label{fig:ed_diagonal}
    \end{figure}

Therefore, the value for $\tilde{\Pi}$ can be approximated by finding the turning point $p$ between two Steiner points (which are projections of $u$ and $v$ onto their corresponding diagonal $\tau$) before which we use diagonal walks and after which we use staircase walks. We pre-computes these values between each pair of steiner points in the beginning after constructing the graph. This can be done by computing the values on the 0-th level diagonal, and compute the values on any $i$-th level diagonal using its $i-1$-th level parent diagonal, as shown by Equation \ref{eq:lambda}. 

To prove the correctness, we use the analogous proof of \ref{lemma:diag_weight}. For any diagonal segments $(u, v)$ on the $k+1$-th level diagonal $\tau$, there is a direct line of sight to a corresponding segment $(u', v')$ on a $k$-th level diagonal $\tau'$. The only place where the distance can differ between the two segments is at the sample points $u$ and $u'$. Using the definition of edit distance, we obtain a variant of Equation \ref{eq:lambda}:

\begin{equation}
\lambda(u, v) = \lambda(u', v') - \min\{d(u'), 2g\} + \min\{d(u), 2g\}
\label{eq:ed_lambda}
\end{equation}
\end{comment}


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

\paragraph{Motivation.}
Trajectories are functions from a time interval to $\R^d$, for $d \ge 1$, and they
describe how physical systems change over time.  Trajectories are being inferred
and recorded from numerous sources at an incredible rate and are often
represented as a sequence of points.  These sources include the hundreds of
millions of sensors found in traffic monitoring systems, GPS sensors in cellular
phones, and medical devices, and from scientific experiments and simulations.
Groups of trajectories often exhibit shared structure.  Sometimes this structure
is enforced by physical constraints; GPS units in vehicles seldom leave the
road.  However, this structure may also be present in less expected groups of
trajectories such as those representing the movement of
pedestrians~\cite{ghb-uihmp-08} or hurricanes~\cite{lhw-tcpgf-07}.  Having an
effective way to identify similar portions between a pair of trajectories can
greatly aid in understanding these shared patterns.  In such applications, it is
not enough to merely \emph{quantify} how similar pairs of trajectories are; we
need to compute correspondences between their sample points as well.

\paragraph{Problem statement.}
Let~$P = \langle p_1, \ldots, p_m \rangle$ and~$Q = \langle q_1, \ldots, q_n \rangle$ be two sequences of points in~$\R^d$ for some fixed $d > 1$, drawn from
two curves~$\gamma_P$ and~$\gamma_Q$.
We define a \emph{correspondence} as a pair~$(p_i,q_j)$.
A set $C$ of correspondences is \emph{monotone} if for any pair of correspondences
$(p_i,q_j), (p_{i'},q_{j'})$ with $i' \geq i$ we have $j' \geq j$.
We define the cost of $C$ to be $\sum_{(p,q) \in C} ||pq||$, where $||\cdot||$
is the Euclidean norm.  The similar portions of $P$ and $Q$ are represented by a
set $C$ of monotone correspondences, with the cost of $C$ quantifying the quality of
similarity.
The goal is to compute a monotone set of correspondences with certain properties.
While numerous criteria for computing correspondences have been proposed, we
focus on two, which are widely used, namely dynamic time warping (DTW) and edit
distance.  They have been used for matching speech signals, DNA and protein
sequences, protein backbones, time-series data, GPS trajectories, video
trajectories, etc \cite{rabiner1993fundamentals, WG, EFS, DEKM-book, KKL, MP99, KP00, KR05,
Muller-book, CPBTMPCMC-98}.

DTW computes a monotone set of correspondences in which every point in~$P$
and~$Q$ appears at
least once, and minimizes the sum of distances of corresponding pairs of points.
Formally, the cost of DTW, denoted by $\dtw(P,Q)$, is 
%\begin{equation}
  %\dtw(P,Q) = \min_{C} \sum_{(p,q) \in C} ||pq||,
  %%\label{eq:dtw_def}
%\end{equation}
  $\dtw(P,Q) = \min_{C} \sum_{(p,q) \in C} ||pq||$,
where the minimum is taken over all sets $C$ of monotone correspondences that
cover all points of $P$ and $Q$.
DTW allows a point to appear in multiple correspondences, so it matches two curves effectively
even if the sampling rates are different.

Edit distance (also called Levenshtein distance) seeks a monotone
\emph{matching} on the points in~$P$ and~$Q$ of minimum cost; each point in
$P$ corresponds to at most one point in $Q$ and vice versa.
It also adds an additional constant \emph{gap} penalty~$g$ for each point in~$P
\cup Q$ that
does not appear in a correspondence.
Formally, the cost of the edit distance, denoted by $\ed(P,Q)$, is 
%\begin{equation}
  %\ed(P,Q) = \min_C \sum_{(p,q) \in C} ||pq|| + g(m+n-2|C|),
  %\label{eq:ed_def}
%\end{equation}
  $\ed(P,Q) = \min_C \sum_{(p,q) \in C} ||pq|| + g(m+n-2|C|)$,
where the minimum is taken over all sets $C$ of monotone correspondences that
are matchings in the complete bipartite graph $P \times Q$.  More sophisticated
gap penalty functions have been proposed, but we focus on the simple linear gap
penalty function.
By tuning~$g$ correctly, meaningful correspondences can be computed even when faced with
outlier points that arise from measurement errors or short deviations in otherwise similar
trajectories.

Given a parameter $\eps \in (0,1)$, we wish to develop efficient
$(1+\eps)$-approximation algorithms for computing $\dtw(P,Q)$ and $\ed(P,Q)$,
i.e., they return a value $\Delta$ such that $\dtw(P,Q) \le \Delta \le (1+\eps)
\dtw(P,Q)$ or $\ed(P,Q) \le \Delta \le (1+\eps) \ed(P,Q)$.  We are also
interested in computing correspondences that realize these distances.


\paragraph{Prior results.}
%As the recursive definitions suggest, there are straightforward quadratic time dynamic programming
%algorithms to compute these and other distance measures such as the discrete \frechet
%distance~\cite{ALT1995,Eiter1994}.
%The \emph{discrete \frechet distance} seeks a monotone correspondence which includes every point
%while minimizing the \emph{maximum} pairwise distance between corresponding points\footnote{We
%note that while (discrete) \frechet distance is a reasonable measure to compute the similarity
%between two curves, it is not effective in identifying similar portions of the curves.}.
%Other than a logarithmic factor improvement by Agarwal \etal~in the computation time for
%discrete \frechet distance~\cite{pankaj_discretefr}, these dynamic programming algorithms remain
%the best known for computing their distance measures (see also work by Buchin
%\etal~\cite{Buchin2014} on continuous \frechet distance).
%Bringmann~\cite{Bringmann14SETH} recently provided an explanation for this lack of progress.
It is well-known that both $\dtw(P,Q)$ and $\ed(P,Q)$, as well as the relevant
correspondences, can be computed in $O(mn)$ time using dynamic programming
\cite{KT2005}.
A series of recent papers suggest that 
there exists no algorithm for computing $\dtw(P,Q)$ or $\ed(P,Q)$ in
time~$O(n^{2-\delta})$ for any~$\delta > 0$ unless the Strong Exponential Time Hypothesis (SETH)
of Impagliazzo and Paturi~\cite{Impagliazzo2001} is false.
In particular, Backurs and Indyk~\cite{BI2015} showed a lower bound for edit distance, and
Abboud, Backurs, and Williams~\cite{ABW2015} and Bringmann and K\"unnemann~\cite{BK2015}
independently showed lower bounds for DTW.
While most of these lower bounds were presented for the string versions of their respective
problems, the DTW lower bound of Bringmann and K\"unnemann uses sequences of points in~$\R$.
Unless SETH is false, there exists no strictly sub-quadratic time algorithm for DTW, even in our
setting of point sequences in~$\R^d$.
Similar conditional lower bounds have been shown for other distance and similarity
problems~\cite{AWW2014,BI2015,ABW2015,Bringmann14SETH,BK2015}.
Some of these results suggest that even strongly sub-quadratic approximation
schemes seem unlikely \cite{ABW2015,Bringmann14SETH}.


In view of the recent lower bounds, a natural question to ask is whether
near-linear, or even subquadratic, algorithms exists for certain natural
families of curves.  Aronov
\etal~\cite{AHKWW2006} gave strictly sub-quadratic time approximation schemes for
the discrete \frechet distance of point sequences taken from two families of curves,
called \emph{$\kappa$-bounded curves} and \emph{backbone curves}.
Discrete \frechet distance is similar to DTW except that one uses max instead of
sum.
%in Eq.~(\ref{eq:dtw_def}).
Restricting themselves to these families of curves allowed them to subvert the hardness result of
Bringmann~\cite{Bringmann14SETH} mentioned above.
Driemel, Har-Peled, and Wenk~\cite{DHW2012} extended the approximation results to the continuous
\frechet distance and the even more natural family of \emph{$\kappa$-packed} curves (see
below for definitions of these families of curves);
see also Bringmann and
K\"unnemann~\cite{BK2014} and Bringmann and Mulzer~\cite{BM2015SoCG}.
We note that while (discrete) \frechet distance is a reasonable measure to
compute the similarity between two curves, it is not effective in identifying
similar portions of the curves.

Currently, no approximation results are known for DTW, although there are a number of heuristics
designed to speed up its exact computation in practice; see Wang \etal~\cite{WMDTSK13}.
Approximation algorithms are known for variants of edit distance, but all of these algorithm have
at least a polylogarithmic approximation ratio.
See Andoni \etal~\cite{AKO2010} and the references therein.

\paragraph{Our results.}
\note{Update results and high level description of algorithm.}
We present sampling based algorithms for computing $\dtw(P,Q)$ and $\ed(P,Q)$
approximately, as well as for computing the correspondences realizing these
distances.  The two algorithms are almost identical except a few small details.
In the worst case, their running time is quadratic for arbitrary point
sequences, but it is near-linear when $P$ and $Q$ are drawn from certain natural
families of curves --- these are the first approximation algorithms that compute
$\dtw(P,Q)$ and $\ed(P,Q)$ for such point sequences in subquadratic time.  We
present concrete bounds for two specific families of curves --- $\kappa$-packed,
and $\kappa$-bounded curves.  For $x \in \R^d$ and $r \in \R^+$, let $\ball(x,
r)$ denote the ball of radius $r$ centered at $x$.  Given $\kappa \in \R^+$, a
curve $\gamma$ in $\R^d$ is \emph{$\kappa$-packed} if the length of $\gamma$
inside any ball of radius $r$ is bounded by $\kappa r$ \cite{DHW2012}, and
$\gamma$ is \emph{$\kappa$-bounded} if for any $0 \le t < t' \le 1$, 
$ \gamma[t:t'] \subseteq \ball\left(\gamma(t), \tfrac{\kappa}{2} ||\gamma(t)
\gamma(t')||\right) \cup \ball\left(\gamma(t'), \tfrac{\kappa}{2} ||\gamma(t)
\gamma(t')||\right),$
where $\gamma: [0,1] \rightarrow \R^d$ and $\gamma[t:t']$ is the portion of
$\gamma$ between $\gamma(t)$ and $\gamma(t')$ \cite{AKW2004}. $\gamma$
See Figure~\ref{fig:alg}(a) and (b).

\begin{theorem}
  Let $P$ and $Q$ be two point sequences of length at most $n$ drawn from
  $\kappa$-packed curves in $\R^d$ for some $\kappa > 0$, and let $\eps \in (0,1)$ be
  a parameter.  Then $O(\frac{\kappa}{\eps} n\log^2n)$-time
  $(1+\eps)$-approximation algorithms exist for computing $\dtw(P,Q)$ and
  $\ed(P,Q)$ and the correspondences that realize these
  distances.
  \label{thm:packed}
\end{theorem}

\begin{theorem}
  Let $P$ and $Q$ be two point sequences of length at most $n$ drawn from
  $\kappa$-bounded curves in $\R^d$ for some $\kappa > 0$, and let $\eps \in (0,1)$ be
  a parameter.  Then $O(\frac{\kappa^d}{\eps^d} n\log^2n)$-time
  $(1+\eps)$-approximation algorithms exist for computing $\dtw(P,Q)$ and
  $\ed(P,Q)$ and the correspondences that realize these
  distances.
  \label{thm:bounded}
\end{theorem}


The framework used to create these algorithms is quite general and yields
near-linear approximation algorithms for
a variety of similar distance measures based on monotone correspondences.
For example, our results immediately generalize to variants of dynamic time warping and
edit distance that use the $k$th powers of distance between points instead of their
Euclidean distance for any constant $k > 0$.  It also yields a subquadratic
algorithm for backbone curves.

A protein backbone curve is commonly used to model protein backbones where each vertex represents a 
$C_\alpha$ atom, connected to its neighbors via covalent bonds. A backbone curve $\gamma$ has the 
following properties: (1) for any pair of vertices $u, v \in \gamma$, $d(u, v) \ge 1$ due to the 
presence of van der Waal interactions; (2) for any pair of consecutive vertices, the covalent bonds
between them has constrained length, i.e. $d(u, v) \in [c_1, c_2]$ \cite{AHKWW2006}.

\begin{theorem}
  Let $P$ and $Q$ be two point sequences of length at most $n$ drawn from
  protein backbone curves in $\R^d$, and let $\eps \in (0,1)$ be
  a parameter.  Then $O(\frac{1}{\eps} n^{2-1/d} \log n)$-time
  $(1+\eps)$-approximation algorithms exist for computing $\dtw(P,Q)$ and
  $\ed(P,Q)$ and the correspondences that realize these
  distances.
  \label{thm:backbone}
\end{theorem}


Recall that the standard dynamic programming algorithm for computing $\dtw(P,Q)$
or $\ed(P,Q)$ constructs a weighted grid DAG $\G$ on $\V = \{(i,j) \mid 1\le i
\le m, 1\le j \le n\}$ and formulates the problem as computing a minimum-weight
path from $s=(1,1)$ to $t=(m,n)$.  Our main idea is to view $\G$ as a
geometric graph embedded on an integer grid in $\R^2$, where one can walk
along horizontal, vertical, or diagonal (slope 1) segments.
By taking a geometric view, we are able to deploy geometric techniques and partition~$\V$ into a
number of rectangles where the points within a rectangle all have similar weight.
Using the geometry of point sequences $P$ and $Q$ and of the curves $\gamma_P$ \& $\gamma_Q$ from
which $P$ and $Q$ are drawn, we show how to choose the rectangles so that the number of boundary
points is near linear when $\gamma_P$ and $\gamma_Q$ are $\kappa$-packed or $\kappa$-bounded.
We then describe an efficient procedure to compute minimum-weight paths to each boundary point
after equalizing the weight of points within each rectangle.

We first describe the algorithm for DTW (Section~\ref{sec:alg}), and then give the procedure to
compute minimum-weight paths (Section~\ref{sec:shortest_paths}).
Next, we analyze the performance of our algorithm (Section~\ref{sec:analysis}), and finally adapt
it to computing edit distance (Section~\ref{sec:ED}).
Section~\ref{sec:clustering} describes the procedure for computing the rectangles
partitioning~$\V$.


==> shortest_paths.tex <==
\section{Computing shortest paths}
\label{sec:shortest_paths}

For a point~$p \in \V$, let~$\chi(p)$ be the minimum cost of a path in~$\G$ from~$s$ to~$p$ under
the cost function~$\lambda$.
For simplicity, we describe the algorithm for computing~$\chi(p)$ for all~$p \in \boundaries$.
The minimum-cost paths can be recovered using standard techniques.

Initially, we set~$\chi(s) = 0$.
We process the rectangles of~$\rects$ in the order computed above.
Suppose we have processed~$\rect_1,\dots,\rect_{u-1}$, i.e. we have computed~$\chi(p)$ for all~$p
\in \boundaries_{u-1} = \Cup_{i=1}^{u-1} \partial \rect_i$.
Let ${\rect_u = [a^{-}:a^{+}] \times [b^{-}:b^{+}]}$ be the next rectangle in~$\rects$.
Without loss of generality, assume that~$a^{+}-a^{-} \ge b^{+}-b^{-}$.
We first compute~$\chi(\cdot)$ for points on the left and bottom boundaries of~$\rect_u$ and then
on the right and top boundaries.

\paragraph{Left and bottom boundaries.}
Since~$(i,j)$ has incoming edges from $\Set{(i-1,j-1),(i-1,j), (i,j-1)}$, we have $\chi(i,j) =
\min \Set{(\chi(i-1,j-1) +
\lambda(i-1,j-1),\chi(i,j-1)+\lambda(i,j-1),\chi(i-1,j)+\lambda(i-1,j-1)}$.
For ${(i,j) = (a^{-},b^{-})}$, all three incoming neighbors belong to~$\boundaries_{u-1}$,
so~$\chi(a^{-},b^{-})$ can be computed in~$O(1)$ time.
For a point $(a^{-},j)$ with~$j \in [b^{-}:b^{+}]$, we have~$(a^{-}-1,j-1),(a^{-},j-1) \in
\boundaries_{u-1}$.
So each~$\chi(a^{-},j)$, for~$j \in [b^{-}:b^{+}]$, can be computed in~$O(1)$ time by iteratively
increasing the value of~$j$.
Similarly,~$\chi(i,b^{-})$, for~$i \in [a^{-}:a^{+}]$, can be computed in~$O(1)$ time each.
Hence, left and right boundaries of~$\rect_u$ can be processed in a total of~$O(|\partial
\rect_u|)$ time.\\

Since~$\lambda(\cdot)$ is the same for all points in~$\rect_u$, the cost of a path~$\pi$ lying
inside~$\rect_u$ is~$\ell(\pi) \lambda \rect_u$.
For a point~$p \in \rect_u$, let~$N(p) \subseteq \partial \rect_u$ be the set of boundary points
of~$\rect_u$ that are strictly dominated by~$p$, i.e., there is a path in~$\G$ from every point
of~$N(p)$ to~$p$.
For two points~$p = (i,j)$ and~$q = (i',j')$ in~$\rect_u$ with~$i' \ge i$ and~$j' \ge j$, the
minimum length of a path from~$p$ to~$q$ is $d(p,q) = \max\Set{i'-i,j'-j}$, and therefore the
minimum cost of a path from~$p$ to~$q$ is~$d(p,q) \lambda \rect_u$.
Hence, for any point~$p$ on the right or top boundary of~$\rect_u$,
$$\chi(p) = \min_{q \in N(p)} \chi(q) + d(q,p) \lambda \rect_u.$$

\paragraph{Right boundary.}
For~$j \in [b^{-}:b^{+}]$, let~$p_j = (a^{+}, j)$ be a point on the right boundary of~$\rect_u$.
We partition~$N(p_j)$ into three sets.
\begin{enumerate}[(i)]
  \item $N_1(p_j) = \Set{(a^{-},l) \mid l \in [b^{-}:j]}$.
    For all points~$q \in N_1(p_j)$, we have~$d(q,p_j) = a^{+} - a^{-}$.
    For~$j \in [b^{-}:b^{+}]$, let~$Q_j = \min_{l \leq j} \chi(a^{-},l)$.
    Therefore,
    $$\min_{q \in N_1(p_j)} \chi(q) + d(q,p_j) \lambda \rect_u = \min_{q \in N_1(p_j)}
    \chi(q) + (a^{+} - a^{-})\lambda \rect_u = Q_j + (a^{+} - a^{-})\lambda \rect_u.$$

  \item $N_2(p_j) = \Set{(i,b^{-}) \mid i \in [a^{-}:a^{+} - (j-b^{-})]}$.
    There is a shortest path from~$q \in N_2(p_j)$ consisting of the horizontal segment $q
    \bar{p}_j$, where $\bar{p}_j = (a^{+} - j + b^{-},b^{-})$, and the diagonal $\bar{p}_j p_j$.
    Hence,
    $$\min_{q \in N_2(p_j)} \chi(q) + d(q,p_j) \lambda \rect_u = \chi(\bar{p_j}) + (j-b^{-})
    \lambda \rect_u.$$

  \item $N_3(p_j) = \Set{(i,b^{-}) \mid i \in [a^{+} - j + b^{-} + 1:b^{+}]} \cup \Set{(a^{+},l
    \mid l \in [b^{-}:j-1]}$.
    There is a shortest path from ${q \in N_3(p_j)}$ to~$p_j$ consisting of the (possibly empty)
    diagonal from~$q$ followed by a vertical segment on the right boundary of~$\rect_u$.
    In particular, it passes through~$p_{j-1}$.
    Hence,
    $$\min_{q \in N_3(p_j)} \chi(q) + d(q,p_j) \lambda \rect_u = \chi(p_{j-1}) + \lambda
    \rect_u.$$
\end{enumerate}

Putting everything together,
\begin{align*}
\chi(p_j) &= \min_{q \in N(p_j)} \chi(q) + d(q,p_j) \lambda \rect_u \\
  &= \min\Set{Q_j + (a^{+}-a^{-}) \lambda \rect_u,\chi(\bar{p}_j) + (j-b^{-}) \lambda \rect_u,
  \chi(p_{j-1}) + \lambda \rect_u}.
\end{align*}

By making a pass through the left boundary of~$\rect_u$, value~$Q_j$, for~$j \in [b^{-}:b^{+}]$,
can be computed in a total of~$O(b^{+}-b^{-})$ time.
After having computed~$Q_j$'s,~$\chi(p_j)$ can be computed in~$O(1)$ time each.

\paragraph{Top boundary.}
For $i \in [a^{-}:a^{+}]$, let $p_i = (i, b^{+})$ be a point on the top boundary of~$\rect_u$.
There are two cases whether the diagonal segment passing through~$p_i$ intersects the left or the
bottom boundary of~$\rect_u$, i.e. whether $i \le b^{+} - b^{-} + a^{-}$.
\paragraph{Case: $i \le a^{-} + (b^{+} - b^{-})$.}
This case is symmetric to the right boundary case.
We partition~$N(p_i)$ into three parts.
\begin{enumerate}[(i)]
  \item $N_1(p_i) = \Set{(a^{-}, j) \mid j \in [b^{-} + 1:b^{+} - i + a^{-}]}$.
    For $q \in N_1(p_i)$, there is a shortest path from~$q$ to~$p_i$ that passes
    through~$p_{i-1}$.
    Hence,
    $$\min_{q \in N_1(p_i)} \chi(q) + d(q,p_i) \lambda \rect_u = \chi(p_{i-1}) + \lambda
    \rect_u.$$

  \item $N_2(p_i) = \Set{(a^{-}, j) \mid j \in [b^{-}:b^{+} - i + a^{-}]}$.
    For $q \in N_2(p_i)$, there is a shortest path from~$q$ to~$p_i$ that passes through
    $\bar{p}_i = (a^{-}, b^{+} - i + a^{-})$, the intersection point of the diagonal through~$p_i$
    with the left boundary of~$\rect_u$.
    Hence,
    $$\mid_{q \in N_2(p_i)} \chi(q) + d(q,p_i) \lambda \rect_u = \chi(\bar{p}_i) + (i -
    a^{-}) \lambda \rect_u.$$

  \item $N_3(p_i) = \Set{(l, b^{-}) \mid l \in [a^{-}, i]}$.
    Let $\psi_i = \min_{a^{-} \le l \le i} \chi(l, b^{-})$.
    For any $q \in N_3(p_i)$, we have $d(q,p_i) = b^{+}-b^{-}$.
    Therefore,
    $$\min_{q \in N_3(p_i)} \chi(q) + d(q,p_i) \lambda \rect_u = \psi_i + (b^{+} - b^{-}) \lambda
    \rect_u.$$
\end{enumerate}

Hence,
$$\chi(p_i) = \min\Set{\chi(p_{i-1}) + \lambda \rect_u, \chi(\bar{p}_i) + (i-a^{-}) \lambda
\rect_u, \psi_i + (b^{+} - b^{-}) \lambda \rect_u}.$$

As for the right boundary, after computing~$\psi_i$, for $i \in [a^{-}: a^{-} + (b^{+} - b^{-})]$,
we can compute~$\chi(p_i)$, for each $i \in [a^{-}:a^{-} + (b^{+} - b^{-})]$ in~$O(1)$ time each.

\paragraph{Case: $i > a^{-} + (b^{+} - b^{-})$.}
We partition~$N(p_i)$ into two sets.
\begin{enumerate}[(i)]
  \item $N_1(p_i) = \Set{(a^{-},j) \mid j \in [b^{-}:b^{+}]} \cup \Set{(l,b^{-}) \mid l \in
    [a^{-}:i-b^{+} + b^{-} - 1]} \cup {(l,b^{+}) \mid l \in [a^{-}:i-1]}$.
    For all $q \in N_1(p_i)$, there is a shortest path from~$q$ to~$p_i$ that passes
    through~$p_{i-1}$.
    Hence,
    $$\min_{q \in N_1(p_i)} \chi(q) + d(q,p_i) \lambda \rect_u = \chi(p_{i-1}) + \lambda
    \rect_u.$$
  \item $N_2(p_i) = \Set{(l,b^{-}) \mid l \in [i - b^{+} - b^{-}:i]}$.
    For all $q \in N_2(p_i)$, we have $d(q,p_i) = b^{+} - b^{-}$.
    Therefore,
    $$\min_{q \in N_2(p_i)} \chi(q) + d(q,p_i) \lambda \rect_u = \tilde{\psi}_i + (b^{+} - b^{-})
    \lambda \rect_u$$
    where $\tilde{\psi}_i = \min_{q \in N_2(p_i)} \chi(q)$.
\end{enumerate}

Hence,
$$\chi(p_i) = \min\Set{\chi(p_{i-1}) + \lambda \rect_u, \tilde{\psi}_i + (b^{+} - b^{-}) \lambda
\rect_u}.$$
Note that for $i > a^{-} + (b^{+} - b^{-})$, we have $N_2(p_{i+1}) = (N_2(p_i) \cup \Set{(i+1,
b^{-})}) \setminus \Set{(i - b^{+} - b^{-}, b^{-})}$.
That is, computing~$\tilde{\psi}_i$'s requires maintaining the minimum of the set of items in a
`window' of length $b^{+} - b^{-}$ as we slide the window.
This task can be accomplished as follows.
We maintain a subsequence $Q = \langle p_{i1}, \dots, p_{ir} \rangle$ of items such that (i)
$\chi(p_{i l}) < \chi(p_{i(l + 1)})$ for $1 \le l \le r$, and (ii) for all $b \in [il+1:i(l+1) -
1]$, we have $\chi(p_b) \ge \chi(p_{i(l+1)})$.
Then, $\tilde{\psi}_i = \chi(p_{i1})$.

When we process~$p_{i+1}$, we remove~$p_{i1}$ from~$Q$ if~$i1 = i + 1 - b^{+} - b^{-}$.
Next, we scan~$Q$ backwards and remove the current item~$p_{il}$ being scanned if $\chi(p_{il})
\geq \chi((i+1,b^{-}))$.
Finally, we insert $(i+1,b^{-})$ into~$Q$ as its last item.
The time spent in updating~$Q$ while processing~$p_i$ is~$O(1+\kappa_i)$ where~$\kappa_i$ is the
number of items deleted from~$Q$ while processing~$p_i$.
Since each item is deleted at most once, the total running time is~$O(a^{+} - a^{-})$.

Putting everything together, the total time spent processing~$\rect_u$ is~$O(|\partial \rect_u|)$.
Hence, we conclude the following.
\begin{lemma}
  The total time spent in computing~$\chi(p)$ for all points $p \in \boundaries$ is~$O(\beta)$.
\end{lemma}

